Multiparty Classical Choreographies

We present Multiparty Classical Choreographies (MCC), a language model where global descriptions of communicating systems (choreographies) implement typed multiparty sessions. Typing is achieved by generalising classical linear logic to judgements that explicitly record parallelism by means of hypersequents. Our approach unifies different lines of work on choreographies and processes with multiparty sessions, as well as their connection to linear logic. Thus, results developed in one context are carried over to the others. Key novelties of MCC include support for server invocation in choreographies, as well as logic-driven compilation of choreographies with replicated processes.

==> cc.tex <==
In this section we formally present Multiparty Classical
Choreographies (MCC). We begin by introducing its {\em action
  fragment}, a variant of Globally-governed Classical Processes
(GCP)~\cite{CLMSW16}. We then continue by extending GCP to MCC.

% We present Multiparty Classical Choreographies (MCC), a language
% model allowing modular composition of choreographies and processes. We
% begin by presenting the syntax of programs, program types and global
% types of sessions. We continue by giving the proof theory of MCC,
% which includes rules for typing of processes and choreographies, as
% well as a judgment for verifying that types used in a communication
% are compatible (coherent).


\subsection{GCP with hypersequents} 
\paragraph{Syntax.} GCP is a generalization of Classical
Process~\cite{W12} that deals with multiparty session types. As hinted
in \S~\ref{sec:preview}, when writing a program in our language, we do
not identify sessions via channel names, but rather we name sessions'
\emph{endpoints}. Each process owns a single endpoint of a session it
participates in. The complete syntax of GCP is given by the following
grammar:
% \begin{align*}\small
%   P ::= & \rule{3mm}{0mm}
%   \hl{\axiom{x}{A}{y}{B}} 
%    \mid   \hl{ P\pp Q}     
%    \mid \hl{\res {{\til x}:G} P}    
%    \mid \hl{\gensend}     
%    \mid \hl{\genrecv}    
%    \mid \hl{\genclose}    \\
%   &\mid \hl{\genwait}     
%    \mid \hl{\geninl}      
%    \mid \hl{\gencase}     
%    \mid \hl{\geninr}      
%    \mid \hl{\geninlinr}   
%    \mid \hl{\genclient}   \\
%   &\mid \hl{\gensrv}      
%    \mid \hl{\genshutdown}
%    \mid \hl{\genclone}    
%    \mid \hl{\gensendt}   
%    \mid \hl{\genrecvt}   
%    \mid \hl{\gennocase}  
% \end{align*}
\begin{displaymath}\scriptsize
  \begin{array}{rll@{\qquad\qquad}llllllllll}
    P ::= & \rule{1.4mm}{0mm}
    \hl{\axiom{x}{A}{y}{B}} & \text{link} 
    & \mid \hl{\genclient} & \text{client}
    \\
    & \mid \hl{ P\pp Q}     & \text{parallel}
    & \mid \hl{\gensrv}& \text{server}
    \\
    & \mid \hl{\res {{\til x}:G} P} & \text{restriction}
    & \mid \hl{\genshutdown} & \text{server kill}
    \\
    & \mid \hl{\gensend} & \text{send}
    & \mid \hl{\genclone}    & \text{server clone}
    \\
    & \mid \hl{\genrecv} & \text{receive}
    & \mid \hl{\gensendt} & \text{send type}
    \\
    & \mid \hl{\genclose} & \text{close session}
    & \mid \hl{\genrecvt} & \text{receive type}
    \\
    & \mid \hl{\genwait} & \text{receive close}
    & \mid \hl{\gencase} & \text{branching}
    \\
    & \mid \hl{\geninl} & \text{left selection}
    & \mid \hl{\geninlinr} & \text{general selection}
    \\
    & \mid \hl{\geninr} & \text{right selection}
    & \mid \hl{\gennocase} & \text{empty choice}
%     \\
%     & \mid \hl{\genclient}   &
%   & \mid \hl{\gensrv}      &
%   &  && \text{server accept/request}\\
% %
%   & \mid \hl{\genshutdown} &
%   &&
%   & && \text{server kill}\\
% %
%   & \mid \hl{\genclone}    &
%   &&
%   &   && \text{server clone}\\
% %
%   & \mid \hl{\gensendt}    &
%   & \mid \hl{\genrecvt}    &
%   &     && \text{type communication}\\
% %
%   & \mid \hl{\gennocase}   &&&&&& \text{empty choice}
  \end{array}
\end{displaymath}
%
With a few exceptions, the terms above are identical to those of
GCP. For space restriction reasons, we only discuss the key
differences.  Among the structural constructs, we have separated
parallel composition from the restriction operator.  We further allow
the non-deterministic selection $\geninlinr$, denoting a process that
non-deterministically selects a left or a right branch.
%
For services, an endpoint $x$ may kill all the servers by executing
the action $\genshutdown$, or duplicate them by means of $\genclone$
-- these operations were silent in the original CP and GCP
presentations. In the last case, the new copies of the servers are
replicated at fresh endpoints, and are ready to engage in a session
with endpoint $x'$.

Types are defined as follows:
{\scriptsize
\begin{align*}
A ::= & \rule{3mm}{0mm}\hl{A\tensor B}       && \text{output} &
  & \mid \hl{A\parr B}        && \text{input} & \
G ::= & \rule{3mm}{0mm}\hl{\gcom {\til x}{y}{G};H}  && (\tensor\parr)\\
%
  & \mid \hl{A\oplus B}       && \text{selection} &
  & \mid \hl{A\with B}             && \text{choice} &
  & \mid \hl{\gsel x{\til y}{G}{H}} && (\oplus\with) \\
%
  & \mid \hl{!A}                  && \text{server} &
  & \mid \hl{?A}             && \text{client} &
  & \mid \hl{\gbang{x}{\til y}{G}}  && (!?) \\
%
  & \mid \hl{\one}              && \text{close} &
  & \mid \hl{\bot}         && \text{wait} &
  & \mid \hl{\gclose{\til x}{y}} && (\one\bot) \\
%
  & \mid \hl{0}          && \text{false} &
  & \mid \hl{\top}             && \text{empty} &
  & \mid \hl{\gabsurd{x}{\til y}}      && (0\top) \\
%
  & \mid \hl{\forall X.A}       && \text{send type} &
  & \mid \hl{\exists X.A} && \text{receive type} &
  & \mid \hl{\gtypecom {X}{x}{\til y}{G}} && (\exists\forall) \\
%
  & \mid \hl{X} && \text{variable} &
  & \mid \hl{X^\bot} && \text{dual variable} &
  & \mid \hl{\globalaxiom{x}{A}{y}{B}}             && (\textsc{axiom})
\end{align*}
}% Types are used to ensure proper behaviour of participants in a
session. In the multiparty setting, these can be split into
\emph{local types} $A$, which specify behaviours of a single process,
and \emph{global types} $G$, which describe interaction within
sessions (and choreography actions). Again most global types
correspond to pairs of local types, the exception being the global
axiom type, describing a linking session.  Local type operators are
based on connectives from classical linear logic -- thus, ${A\tensor
  B}$ is the type of a process that outputs an endpoint of type $A$
and continues with type $B$, whereas ${A\parr B}$ is the type of a
process that receives endpoints of type $A$ and is itself ready to
continue as $B$. The corresponding global type ${\gcom {\til
    x}{y}{G};H}$ types the choreographic interaction where each of the
processes owning an endpoint $x_i$ sends their new endpoint to
$y$. The exceptions are types $0$ and $0\top$, which are not assigned
to any process ($0$): % or choreography ($0\top$) the inclusion of $0$
is justified by the necessity of having a dual type to $\top$, while
the type $0\top$ is essential for the definition of coherence.  We use
type variables also to represent concrete datatypes.

It is worth noting that the logic formulas in our type system enjoy
the usual notion of duality, where a formula's dual is obtained by
recursively replacing each connective by the other one in the same row
in the table above. For example, the dual of $!(A\tensor0)$ is
$?(A^\bot\parr\top)$, where $A^\bot$ is the dual of formula $A$.

\paragraph{Typing.}
Terms of GCP (and MCC in general) are typed in judgements of the form
$\judge\Sigma P\Psi$, where:
\begin{itemize}
\item $\Sigma$ is a set of session typings of the form
  $\pair{(x_i)_i}{G}$;
\item $P$ is a proof term: a process or a choreography (outside GCP
  fragment);
\item $\Psi$ is a hypersequent: a parallel composition of
  classical linear logic sequents.
\end{itemize}
Intuitively, ${\judge\Sigma P\Psi}$ reads as: $\Psi$ types the program
$P$ under the sessions described in $\Sigma$. Given a judgment $\judge
\Sigma P {\Psi \pp \vdash \Gamma, x : A}$, checking whether $x$ is
\emph{available} -- not engaged in a session -- can be done by
verifying that $x$ does not occur in the domain of $\Sigma$. It should
be noted that names cannot occur more than once in $\Sigma$: each
endpoint $x$ may only belong to (at most) one session
$G$. Hypersequents $\Psi_1, \Psi_2$ and sets of sessions $\Sigma_1,
\Sigma_2$ can only be joined if the names used in their domains do not
repeat.

To separate restriction and parallel composition in our system
(reasons for this separation will be explained in
Sec.~\ref{sec:choreo}), we will have to also split a $\m{Cut}$ rule
known from (linear) logic into two, $\m{Conn}$ and $\m{Scope}$:
{\scriptsize
\begin{align*}
 &\infer[\m{Conn}]
      {
        \judge{(\Sigma_i)_i, \pair{(x_i)_i}{G}}{(P_i)_i}{\left(\Psi_i \pp \seq \Gamma_i, \pair{x_i}{A_i} 
          \right)_i}
      }
      {
        \left(
        \judge{\Sigma_i}{P_i}{\Psi_i \pp \seq \Gamma_i, \pair{x_i}{A_i}}
        \right)_i
        &
        G \gseq (\pair{x_i}{A_i})_i
      }
  &&\quad % \\[1ex]
    &\infer[\m{Scope}]
      {\judge{\Sigma}{\res {{\til x}:G} P}{\Psi \pp \seq \left( \Gamma_i \right)_i}}
      {\judge{\Sigma, \pair{(x_i)_i}{G}}{P}{\Psi \pp \left(\seq \Gamma_i, \pair{x_i}{A_i} \right)_i}}
\end{align*}        
}%
In order for $\m{Conn}$ to establish a connection between processes
$P_i$, we are putting them in parallel. Because the communication has
not been executed yet, we still have to distinguish between the
contexts for each of the endpoints participating in the session --
thus, we use a hypersequent presentation. The sequents involved in a
session get merged once a $\m{Scope}$ rule is applied. This
hypersequent presentation is similar to a classical linear logic
variant of \cite{CMS18} with sessions explicitly remebered in a
separate context $\Sigma$. This is merely a technical device, useful
in a presentation with endpoints.

\input{figures/coherence} When describing a multiparty session, simple
duality of types does not suffice to talk about their
compatibility. Instead, like in \cite{CLMSW16}, we rely on the notion
of \emph{coherence} -- denoted $G \gseq (\pair{x_i}{A_i})_i$ in the
premise of the $\m{Conn}$ rule. In Fig.~\ref{fig:coherence}, we report
the rules defining the coherence relation $\gseq$. We do not describe
these here in detail, as they do not change compared to the original
GCP presentation.

We give the complete presentation of the action fragment of our system
using hypersequents on Fig.~\ref{fig:mcc_action} in
Appendix~\ref{sec:app}, focusing here on giving a flavour of this part
by showing some selected rules:

{\scriptsize
\[\begin{array}{lc}
    &\infer[\m{Ax}]
    {
      \judge{\cdot}{\axiom{x}{A}{y}{B}}{\seq \pair xA, \pair yB}
    }
    {
      A^\bot = B
    }
    \\[2ex]
    &\infer[\tensor]
    {
      \judge{\Sigma_1,\Sigma_2}{\gensend}
            {
              \Psi_1\pp
              \Psi_2\pp
              \seq {\Gamma_1,\Gamma_2,\pair x {A\tensort y B}}
            }
    }
    {
      \judge{\Sigma_1} P {\Psi_1\pp\seq {\Gamma_1, \pair{x'}A}}
      &
      \judge{\Sigma_2} Q {\Psi_2\pp\seq {\Gamma_2,\pair xB}}
    }
    \\[2ex]
    &\infer[\parr]
          {
            \judge{\Sigma}{\genrecv}
                  { \Psi\pp \seq {\Gamma, \pair y{A\parrt{\til x} B}} }
          }
          {
            \judge{\Sigma}P
                  {\Psi\pp \seq {\Gamma, \pair{y'}A, \pair yB} }
          }    
  \end{array}\]        
}%
In this fragment, we work with processes not involved in any session
-- the endpoints explicitly mentioned in proof terms can not occur in
the domain of $\Sigma$, and the rules will generally not affect
ongoing sessions (with the exception of $\tensor$ rule presented
above, where existing sessions have to be split among the two
processes, combined in the conclusion of the rule). [MAYBE COMMENT ALL
RULES REPORTED, BUT SAVING SPACE]

\subsection{Extending GCP with choreographies}\label{sec:choreo}
In order to obtain full MCC, we extend the syntax of GCP with
choreography terms. 
\paragraph{Syntax.} % Programs in MCC can be composed of both processes
% and choreographies, resulting in a fully modular design.
Unlike a GCP process, a choreography, which describes a global view of
a communication within a session, will own all of the endpoints of a
session it describes. We extend GCP with the {\em interaction
  fragment} which is defined by the following grammar:
\begin{displaymath}\scriptsize
  \begin{array}{rllllllll}
    P ::= & \rule{1.5mm}{0mm}\ldots\hl{\axiom{x}{A}{y}{B}} & \mid \hl{\genaxcut} & \text{link} \\
          & \mid   \hl{ P\pp Q}       & \text{parallel composition}\\
          & \mid \hl{\res {{\til x}:G} P} & \text{restriction}\\
          & \mid \hl{\gensend} \quad  \mid \hl{\genrecv}  \quad \mid \hl{\gencom} & \text{communication}\\
          & \mid \hl{\genclose} \quad \mid \hl{\genwait}  \mid \hl{\gencomclose}  & \text{session close}\\
          & \mid \hl{\geninl}    \quad \mid \hl{\gencase}     &
%   & \mid \hl{\genginl}     && \text{left selection}\\
% %
%   & \mid \hl{\geninr}      &
%   &&
%   & \mid \hl{\genginr}     && \text{right selection}\\
%   & \mid \hl{\geninlinr}   & & & &
%   \mid \hl{\genchinlinr} && \text{general selection}\\
% %
%   & \mid \hl{\genclient}   &
%   & \mid \hl{\gensrv}      &
%   & \mid \hl{\gengclient}  && \text{server accept/request}\\
% %
%   & \mid \hl{\genshutdown} &
%   &&
%   & \mid \hl{\gengshutdown}&& \text{server kill}\\
% %
%   & \mid \hl{\genclone}    &
%   &&
%   & \mid \hl{\gengclone}   && \text{server clone}\\
% %
%   & \mid \hl{\gensendt}    &
%   & \mid \hl{\genrecvt}    &
%   & \mid \hl{\gencomt}     && \text{type communication}\\
% %
%   & \mid \hl{\gennocase}   &&&&&& \text{empty choice}
\end{array}
\end{displaymath}
The link term $\genaxcut$ gives the choreographic view of an axiom
connected to some other process $P$ through endpoints $x$ and $y$. A
linear interaction $\gencom$ denotes a communication from endpoints
$\til x$ to endpoint $y$, where a new session with endpoints
$\til x'$,$y'$ is created. The choreography $\gencomclose$ closes a
session between endpoints $\til x$, $y$. When it comes to branching,
we have two choreographic terms denoting left and right selection:
$\genginl$ and $\genginr$. A third term, $\genchinlinr$, is used for
non-deterministic choice. In MCC, we can model non-linear behaviour:
this is done with the terms $\gengclient$, $\gengshutdown$ and
$\gengclone$. The first term features a client $x$ starting a new
session with servers $\til y$, while the second term is used by
endpoint $x$ to shut down servers $\til y$. Finally, we have a term
for cloning servers so that they can be used by different clients in
different sessions. The term $\gencomt$ is the choreographic view of a
type communication from an endpoint $x$ to endpoints $\til y$.





\paragraph{Typing.} Fig.~\ref{fig:mcc_interaction} details the rules
for typing choreography terms. At the process level, each of these
rules combines two rules from the GCP fragment. Unlike process rules,
the choreography rules now also look at $\Sigma$ to check that the
interactions described conform to the types of the ongoing sessions.
In rule~$\onebot$, we close a session (removed from $\Sigma$) and
terminate all processes involved in it.  Rule~$\tensorparr$ types the
creation of a new session with protocol $G$, created among endpoints
$\til z$ and $w$; this session is stored in $\Sigma$, while the
process types are updated as in rules~$\tensor$ and $\parr$ above.
The remaining rules in the linear fragment are similarly
understood. Exponentials give rise to three rules, all of them
combining $\bang$ with another rule.  In rule~$\bangwhynot$, process
$x$ invokes the services provided by $\til y$, creating a new session
among these processes with type $G$.  Rule~$\bangw$ combines $\bang$
with $\m{Weaken}$: here the processes providing the service are simply
removed from the context.  Rule~$\bangC$ combines $\bang$ with
$\m{Contract}$, allowing a service to be duplicated.  Finally,
rule~$\existsforall$ allows $x$ to pass values to parameters in
$\til y$, which are then instantiated by a fresh name $A$ throughout
the whole judgement.  \input{figures/mcc_interaction}

%% \subsection{Syntax}\label{sec:syntax}

%% Programs in MCC can be composed of both processes and choreographies,
%% resulting in a fully modular design. When writing a program in our
%% language, we do not identify sessions via channel names, but rather we
%% name sessions' \emph{endpoints}. Each process owns a single endpoint
%% of a session it participates in. %
%% %% A process will then have ownership of
%% %% only one endpoint of a session, but it will be aware of names of its
%% %% other endpoints.
%% By contrast, a choreography, which describes a
%% global view of a communication within a session, will own all of such
%% session's endpoints. The complete syntax of MCC is presented in
%% Fig.~\ref{fig:mcc_syntax}.
%% \input{figures/syntax}

%% The first constructs are structural: a process can be a link between
%% two (compatible) endpoints, a parallel composition of two processes,
%% or
%% a private session among (typed) endpoints $\til{x}$ satisfying the
%% global type $G$.
%% %% , or a choice of two other processes, only one of which will be executed.
%% All remaining constructs come in two flavours:
%% \emph{actions}, executed by a single endpoint of a process (the first
%% two columns), or choreography \emph{interactions} (third column),
%% which specify several actions being executed simultaneously.

%% The actions $\hl \gensend$, $\hl \genrecv$ and $\hl \gencom$ regard
%% session creation, with the process owning endpoint $y$ acting as a
%% coordinator, gathering information about the newly constructed
%% session.  In $\hl \genrecv$, the process owning $y$ waits for the
%% processes joining the new session to each send the new endpoint they
%% plan to use. % in that session.
%% In the newly constructed session, this process will use $y'$ --
%% indeed, it continues as $\hl P$, a process which owns both $y$ and
%% $y'$. Dually, in $\hl \gensend$, the process owning $x$ notifies the
%% coordinator of its intention to join the new session and sends its own
%% endpoint $x'$ for it. In the continuation, $\hl P$ is the protocol for
%% endpoint $x'$ and $\hl Q$ is the protocol for endpoint
%% $x$. Choreographically, we have $\hl \gencom$. % expresses the same
%% % behaviour at a global level.

%% The next constructs model termination of a session. In $\hl \genwait$,
%% the owner of $y$ waits for all other endpoints to execute their $\hl
%% \genclose$ action (and terminate), and then proceeds as $\hl P$. The
%% corresponding choreography is $\hl \gencomclose$.

%% In the case of choice, $\hl \gencase$, endpoint $y$ offers a choice of
%% two possible behaviours; these are selected by a dual selection
%% actions: $\hl \geninl$ or $\hl \geninr$. The selection is the same for
%% all $\til x$ offering a choice. Again, there are corresponding
%% choreographic actions $\hl \genginl$ and $\hl \genginr$.
%% We further allow general selection, $\hl \geninlinr$ in the process
%% form, leaving the decision about the selected branch to be made during
%% execution; a corresponding choreographic action is then $\hl \genchinlinr$.

%% In $\hl \gensrv$, the process owning $y$ offers a service at endpoint
%% $y$ with protocol $\hl P$. This server can react to three kinds of
%% requests.  In the action $\hl \genclient$, endpoint $x$ engages all
%% servers in a session with protocol $\hl P$.  Alternatively, $x$ may
%% kill all the servers by executing the action $\hl \genshutdown$, or
%% duplicate them by means of $\hl \genclone$.  In the last case, the new
%% copies of the servers are replicated at fresh endpoints and are ready
%% to engage in a session with endpoint $x'$. All these behaviours can be
%% invoked by the choreographic actions $\hl \gengclient$, $\hl
%% \gengshutdown$ and $\hl \gengclone$, respectively.  Observe that the
%% choreographic kill action includes the (local) behaviours of all the
%% servers.

%% In the type send action $\hl \gensendt$, $x$ sends type $A$ to
%% processes within its session -- matched by the dual actions $\hl
%% \genrecvt$ for owners of endpoints $y$, receiving the type. This can
%% again be expressed as a choreography $\hl \gencomt$, where $X$ is
%% bound in all actions in $P$ that have $y$ as a subject.

%% Finally, the empty choice $\hl \gennocase$ implements termination,
%% where $\til u$ is a list of dropped endpoints.

%% Types, also defined in Fig.~\ref{fig:mcc_syntax}, are used to ensure
%% proper behaviour of participants in a session. In the multiparty
%% setting, these can be split into \emph{local types} $\hl A$, which
%% specify behaviours of a single process, and \emph{global types} $\hl
%% G$, which describe interaction within sessions and choreography
%% actions. Again most global types correspond to pairs of local types,
%% the exception being the global axiom type, describing a linking
%% session.  Local type operators are based on connectives from classical
%% linear logic -- thus, $\hl{A\tensor B}$ is the type of a process that
%% outputs an endpoint of type $\hl A$ and continues with type $\hl B$,
%% whereas $\hl {A\parr B}$ is the type of a process that receives
%% endpoints of type $\hl A$ and is itself ready to continue as $\hl
%% B$. The corresponding global type $\hl{\gcom {\til x}{y}{G};H}$ types
%% the choreographic interaction where each of the processes owning an
%% endpoint $x_i$ sends their new endpoint to $y$. The exceptions are
%% types $0$ and $0\top$, which are not assigned to any process ($0$) or
%% choreography ($0\top$): the inclusion of $0$ is justified by the
%% necessity of having a dual type to $\top$ (see below), while the type
%% $0\top$ is essential for the definition of coherence (see below).  We
%% use type variables also to represent concrete datatypes.

%% It is worth noting that the logic formulas we use in our type system
%% enjoy the usual notion of duality, where a formula's dual is obtained
%% by recursively replacing each connector by the other one in the same
%% row in Fig.~\ref{fig:mcc_syntax}. For example, the dual of
%% $!(A\tensor0)$ is $?(A^\bot\parr\top)$, where $A^\bot$ is the dual of
%% formula $A$.

%% \subsection{Typing}\label{sec:types}
%% \input{proofsystem}

%% \subsection{Coherence}
%% \input{figures/coherence} In Fig.~\ref{fig:coherence}, we report the
%% rules defining the coherence relation $\gseq$.  These rules follow the
%% intuitions given above, relating global types to their matching
%% choreography actions, when viewed as sets of individual process
%% actions.
%% %In the rule dealing with axioms, endpoints $x$ and $y$ can
%% %communicate only with each other.


%% \subsection{Examples}
%% \todo{remove annot. when final}
%% \paragraph{OpenID.} The OpenID example from \S~\ref{sec:preview} is
%% typable by the global type $G$ (also in \S~\ref{sec:preview}). In
%% particular, we observe that the main endpoints can be typed as:
%% \begin{displaymath}\small
%%   \begin{array}{c}
%%     u:
%%     ?^{rp,ip}(\mathsf{String}^\perp\tensor^{rp}(\mathsf{String^\perp}\tensor^{ip}(\mathsf{Pwd^\perp}\tensor^{ip}
%%     (\mathsf{String^\perp}\tensor^{rp} B))))\\[1mm]
%%     rp:!^u(\mathsf{String}\parr^u ((\mathsf{String}\parr^u C)\&^{ip}
%%                                                                 D_1))\qquad
%%     ip:!^u(\mathsf{String}\parr^u(\mathsf{Pwd}\parr^u (A\oplus^{rp}
%%     D_2)))\\[1mm]
%%     u':
%%     ?^s(\mathsf{String^\perp}\tensor^s(\mathsf{String}\parr^s\perp))\qquad
%%     s:!^{u'}(\mathsf{String}\parr (\mathsf{String^\perp}\tensor^{u'}\one))
%%   \end{array}
%% \end{displaymath}

%% \paragraph{Polymorphism.} In order to show how polymorphic behaviour
%% looks at choreographic level, we recall an example with binary
%% sessions by Wadler~\cite{W14}, which implements Church numerals
%% as polymorphic processes. The parallel composition of a
%% Church numeral with a counter process will return the corresponding
%% natural number, while the composition of a Church numeral with a
%% pinger process will ping the number of times corresponding to such
%% number. We can write such compositions in terms of
%% choreographies. E.g., composing the Church numeral corresponding to
%% one with a counter can be written choreographically as:
%% \begin{displaymath}
%%   \begin{array}{lllll}
%%     \res{xy}\left(
%%     \begin{array}{ll}
%%       \comtype xy{\mathsf{Nat}}X\
%%       \com{x}{s_x}{y}{s_y}\ 
%%       \com{x}{z_x}{y}{z_y}\
%%       \gclient{s_y}{s_x}{}\\
%%       \com{s_x}{a_x}{s_y}{a_y}\
%%       \big(\mathsf{incr}_{a_y,s_y}\pp \mathsf{nought}_{z_x}\pp P\big)
%%     \end{array}\right)
%%   \end{array}
%% \end{displaymath}
%% where $\mathsf{incr}_{a_y,s_y}$ receives a natural number on $a_y$ and
%% sends its successor on $s_y$, while $\mathsf{nought}_{z_x}$ repeatedly
%% outputs zero over $z_x$. Instead, in the case of ping:
%% \begin{displaymath}
%%   \begin{array}{lllll}
%%     \res{xy}\left(
%%     \begin{array}{ll}
%%       \comtype xy{\one}X\
%%       \com{x}{s_x}{y}{s_y}\ 
%%       \com{x}{z_x}{y}{z_y}\
%%       \gclient{s_y}{s_x}{}\\
%%       \com{s_x}{a_x}{s_y}{a_y}{}\ 
%%       \big(\comclose{a_y}{a_x}{}\
%%       \client{w}{v}\ 
%%       \wait{w^{v}}{}\ \comclose{s_x}{s_y}{}\\
%%       \comclose{z_x}{z_y}{}\ 
%%       \comclose{y}{x}{}\ 
%%       \close{u^{u'}}\big)
%%     \end{array}\right)
%%   \end{array}
%% \end{displaymath}
%% where $w$ and $u$ are endpoints used for transmitting the ping to $v$
%% and $u'$.




\begin{remark}[Polymorphism]
  TBD
\end{remark}


% \begin{remark}[Remark on Polymorphism]
%   blah blah
% \end{remark}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> cut_elim.tex <==
% \smallpar{TODO.}
% \begin{enumerate}
% \item Reformulate and refine everything talking about processes and not the 
% proofs, they look weird.
% \item Define a new reduction relation which is up to $\equiv$.
% \end{enumerate}

% In this section, we show the standard result of cut elimination
% applied to our generalised notion of $\m{Cut}$ in MCP, and present
% its consequences.
%
\smallpar{Deadlock Freedom.}  Processes in MCP are guaranteed to be
deadlock-free.
% We the deadlock-freedom property guaranteed by MCP.
We use the standard methodology proposed in~\cite{CP10,W14}.  First, we prove that the $\m{MCut}$
rule in MCP is admissible:
% Below, we write $\DD \pseq \Delta$ to indicate a proof $\DD$ ending
% with judgement $\seq \Delta$. We omit process terms when irrelevant
% for our discussion.
\begin{theorem}[MCut Admissibility]
\label{thm:cut_adm}
  $\hl{P_i} \seq \Gamma_i, \pair {x^{p_i}} {A_i}$, for $i\in[1,n]$,
  and $\hl G \gseq \{\pair{p_i}{A_i}\}_i$ imply that there exists
  $\hl Q$ such that $\hl Q \seq \{\Gamma_i\}_i$.
\end{theorem}
% \begin{proof}
%   By induction on the sizes of the proofs for
%   $\hl{P_i} \seq \Delta_i, \pair {x^{p_i}} {A_i}$ and the formulae
%   $A_i$.
% %
%   If a reduction from Fig.~\ref{fig:mcp_reductions} is applicable,
%   then we apply it. For all such reductions, we can observe that the
%   size of the proof and/or the formulae decrease in the right-hand
%   side, and therefore the thesis follows by induction hypothesis.
% %
%   Otherwise, we can apply one of the commuting conversions from
%   Fig.~\ref{fig:comm_conv}. In this case, the proof gets smaller while
%   the formulas stay the same.
% 
%   Our case coverage is complete, because when a commuting conversion
%   cannot be applied we can always apply a reduction.
%   % We observe that it is never the case that we cannot apply
%   % reductions nor commuting conversions.
%   In fact, commuting conversions cannot be applied only if all proofs
%   for $\hl{P_i}$ end with an application of a rule with principal
%   variable $x$.  But if that is the case, then by coherence we have
%   that there must be at least two proofs for $\hl{P_k}$ and $\hl
%   {P_j}$ that have compatible types and can be reduced.
% \end{proof}

% Theorem~\ref{thm:cut_adm}
The admissibility of $\m{MCut}$ gives us a methodology for removing cuts from a proof, corresponding to executing 
communications in a process
until all restrictions are eventually
eliminated:
\begin{corollary}[Deadlock-Freedom]
  \label{cor:cut_elim}
  $\hl P \seq \Delta$ and $\hl P$ has a restriction imply
  $\hl P \to \hl Q$ for some $\hl Q$.
  % 
  % Then, there exists $\EE$ such that $\EE \pseq \Delta$ and $\EE$
  % has no instances of $\m{Cut}$.
\end{corollary}

\smallpar{Protocol Progress.}
Our correspondence between process and global type reductions goes both ways, a novel result for 
Multiparty Session Types. Below, $\to^+$ denotes one or more 
applications of $\to$:
%
\begin{theorem}[Protocol Progress]
  \label{thm:prot_prog}
  $\hl P \seq \Delta$ and $\gtypes(\hl P) \toglobal \til {\hl{G}}$
  imply $\hl P\to^+ \hl{P'}$ and $\hl {\tilde G} = \gtypes(\hl {P'})$.
  % 
  % % Let $\hl P \seq \Delta$ and $\gtypes(\hl P) \neq \emptyset$.
  % % If $\gtypes(\hl P) \toglobal
  % % \gtypes(\hl{P'})$, then there exists $\hl{P'}$ such that
  % % $\hl P \to^+ \hl{P'}$.
  % CHANGE IT TO: [13/05/2014 11:42:19] Nobuko Yoshida: Assume P |-
  % Delta and gt(P) =/=0.  [13/05/2014 11:43:05] Nobuko Yoshida: Then
  % gt(P) --> G implies there exists P' such that P --> P' and
  % G=gt(P')
\end{theorem}
% Immediately from Corollary~\ref{cor:cut_elim}, we get that MCP
% processes can always normalise and are thus deadlock-free:
% \begin{theorem}[Progress]
%   Let $\hl P$ be a process containing restrictions and such that
%   $\hl P \seq \Delta$. Then, there exists $\hl Q$ such that $\hl P
%   \to \hl Q$ and $\hl Q \seq \Delta$.
% \end{theorem}
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

==> discussion.tex <==
\smallpar{Coherence.}  For the sake of clarity, we made some design
choices in the formalisation of coherence that can be easily
generalised. Some examples are: (i) the $\tensor$ and $\parr$
connectives could be extended to support an arbitrary number of types
on the left-hand and right-hand sides, making them commutative as in
standard linear logic; (ii) rule $!?$ in Fig.~\ref{fig:coherence}
could allow for having some services and some clients rather than
exactly one client; and (iii), similarly, rule $\one\bot$ in
Fig.~\ref{fig:coherence} could be relaxed to allow for more than one
$\bot$ type.  We leave these extensions as interesting future work.
Our choices influence greatly, among other things, the complexity of
the cut admissibility proof for MCP (Theorem~\ref{thm:cut_adm}).  For
example, applying point (iii) would imply that a principal cut
reduction on a terminated session could lead to having more than one
process in the reductum (all the processes typed with $\bot$), whereas
now we have only one. This means that we would have to type a parallel
composition of processes without restriction, which would require to
extend our framework in the fashion of the logic presented
in~\cite{M13:phd}. While extending the proof theory of MCP would be
easy (using, e.g., a notion of partial coherence for typing parallel
composition as done in~\cite{MY13}), it would also cause an explosion
in the number of cases to consider in the proof (see~\cite{M13:phd}
for details).

\smallpar{Identity Axiom in MCP.}
In~\cite{W14}, Wadler shows how the identity axiom of classical linear logic corresponds to a forwarder in the $\pi$-calculus.
We conjecture that the identity axiom can be generalised from using duality to using coherence, by extending our environments in MCP to allow for multiple types for the same session. We left this extension out for a simpler presentation. An example of how the rule could look is:
\begin{displaymath}
\infer[\m{Ax}]
{\hl{\fwd xy} \seq
\pair x{\vec{A[p]}},
\pair y{\vec{B[q]}} 
}
{\hl G \gseq \vec{A[p]},\vec{B[q]}}
\end{displaymath}

\smallpar{Quantifiers.}
The works~\cite{W12,CPPT13} show how to extend session types with existential and universal quantifiers to allow for behavioural polymorphism. We believe that similar extensions can be seamlessly applied to our framework.

\smallpar{Global Types.}
The syntax of our global types is inspired from the works~\cite{HYC08,BCDLDY08}. We added the possibilities of nesting global types and repeating them ($\hl{!G}$); both additions arise naturally from the fact that we based our development on linear logic. Our nesting of global types can be seen as a logical reconstruction of (a simplification of) those originally presented in~\cite{DH12}, where repetitions in global types reconstruct the concept presented in~\cite{CITATION_MISSING}. 


==> figures/eta_expansion.tex <==
\begin{figure*}
  \[
  \begin{array}{lrlr}
    \multicolumn{4}{l}{\textbf{Variables and Local Types:}}\\[1mm]
    \etaexpA {\axiom{x}{A \tensor B}{y}{C \parr D}} & = &
    \recv{y}{x'}{y'}{\send{x}{x'}{y'}{\etaexpA{\axiom{x'}{A}{y'}{C}}}
        {\etaexpA{\axiom{x}{B}{y}{D}}}} & \mbox{for fresh $x',y'$}\\
    \etaexpA{\axiom{x}{\one} {y} {\bot}} & = &
    \wait{y}{\close{x}}\\
    \etaexpA{\axiom{x}{A\oplus B}{y}{C \with D}} & = &
    \Case{y}{\inl{x}{\etaexpA{\axiom{x}{A}{y}{C}}}}{\inr{x}{\etaexpA{\axiom{x}{B}{y}{D}}}}\\
    \etaexpA{\axiom{x}{\bang A}{y}{\quest B}} & = &
    \srv{x}{v}{\client{y}{\til z}{\etaexpA{\axiom{x}{A}{y}{B}}}}\\
    \etaexpA{\axiom{x}{0}{y}{\top}} &=&
    \nocase{y}{v}{} \\
    \etaexpA{\axiom{x}{\exists X.A} y{\forall X.B}} & = &
    \recvtype{y}{v}{X}{\sendtype{x}{\til z}{X}{\etaexpA{\axiom{x}{A}{y}{B}}}}\\
    \etaexpA{\axiom x X y {\dual X}} &= & \axiom x X  y {\dual X}\\
    \etaexpA{\axiom x {\dual X} y{ X}} &= &\axiom x {\dual X} y { X}\\[0.8em]
    
    \multicolumn{4}{l}{\textbf{Global Types:}}\\[1mm]
    \etaexpG {\axiom{x}{A \tensor B}{y}{C \parr D}} & = & {\gcom{x}{y}{\etaexpG{\axiom x A y C}}; {\etaexpG{\axiom x B y D}}}\\
    \etaexpG{\axiom x {\one}y {\bot}} & = & \gclose{x}{y}\\
    \etaexpG{\axiom x {A\oplus B}  y {C \with D}} & = & \gsel{x}{y}{\etaexpG{\axiom x A y C}}{\etaexpG{\axiom x B y D}} \\
    \etaexpG{\axiom x {\bang A} y {\quest B}} & = & \gbang{x}{y}{\etaexpG{\axiom x A y B}}\\
    \etaexpG{\axiom x {0} y{\top}} &=&\topzero{x}{y}\\
    \etaexpG{\axiom x {\exists X.A} y {\forall X.B}} & = & \forallexists{X}{x}{y}{\etaexpG{\axiom x A y B}} \\
    \etaexpG{\axiom x X y {\dual X}} &= & \axiom x X y {\dual X}\\
    \etaexpG{\axiom x {\dual X} y { X}} &= & \axiom x{\dual X} y{ X}\\
      \end{array}
%      \vspace{3mm}
%      \\  
      \] 
%      \vspace*{-2em}
      \caption{$\eta$-expansion}
%      \vspace*{-1em}
      \label{fig:eta_exp_local}
  \end{figure*}


==> figures/mcc_action.tex <==
\begin{figure*}[!hbt]%\scriptsize
  \centering 
  \begin{eqnarray*}
    &\infer[\tensor]
    {
      \judge{\Sigma_1,\Sigma_2}{\gensend}
            {
              \Psi_1\pp
              \Psi_2\pp
              \seq {\Gamma_1,\Gamma_2,\pair x {A\tensort y B}}
            }
    }
    {% Rule Premise below
      \judge{\Sigma_1} P {\Psi_1\pp\seq {\Gamma_1, \pair{x'}A}}
      &
      \judge{\Sigma_2} Q {\Psi_2\pp\seq {\Gamma_2,\pair xB}}
    }
    \\[1ex]
    &\infer[\parr]
          {
            \judge{\Sigma}{\genrecv}
                  { \Psi\pp \seq {\Gamma, \pair y{A\parrt{\til x} B}} }
          }
          {
            \judge{\Sigma}P
                  {\Psi\pp \seq {\Gamma, \pair{y'}A, \pair yB} }
          }
    \\[1ex]
    &\infer[\one]
           {\judge{\cdot}{\genclose} {\seq \pair x {\onet y}}}
           {}
    \qquad
    \infer[\bot]
          {
            \judge{\Sigma}{\genwait}
                  {\Psi\pp \seq \Gamma, \pair y {\bott {\til x}}}
          }
          {
            \judge \Sigma {P}
                   { \Psi\pp \seq \Gamma }
          }
    \\[1ex]
    &\infer[\oplus_1]
        {
          \judge{\Sigma}{\geninl}
                {\Psi \pp \seq \Gamma, \pair {x}{A\oplust{\til y} B}}
        }
        {
          \judge \Sigma P 
                 {\Psi \pp \seq \Gamma, \pair {x}{A}}
        }
    \qquad
    \infer[\oplus_2]
        {
          \judge\Sigma{\geninr} 
                {\Psi \pp \seq \Gamma, \pair {x}{A\oplust{\til y} B}}
        }
        {
          \judge\Sigma Q
                 {\Psi \pp \seq \Gamma, \pair {x}{B}}
        }
    \\[1ex]
      &\infer[\oplus]
        {\judge{\Sigma}{\inlinr{x}{P}{Q}}{\Psi \pp \seq \Gamma, \pair {x}{A\oplus B}}}
        {\judge{\Sigma}{P}{\Psi \pp \seq \Gamma, \pair x A} &
          \judge{\Sigma}{Q}{\Psi \pp \seq \Gamma, \pair x B}}
      \\[1ex]
    &\infer[\with]
      {
        \judge{\Sigma}{\gencase} 
              {\Psi \pp \seq {\Gamma, \pair {y}{A\witht{x} B}}}
      }
      {
        \judge\Sigma P {\Psi \pp  \seq \Gamma, \pair {y}{A}}
        &
        \judge\Sigma Q {\Psi \pp \seq \Gamma, \pair {y}{B}}
      }
      \\[1ex]
    &\infer[!]
      {
        \judge \cdot {\gensrv}
               { \seq {?\Gamma}, \pair {y}{\bang A} }
      }
      {
        \judge \cdot {P}
               { \seq {?\Gamma}, \pair {y}{A} }
      }
    \qquad
    \infer[?]
          {
            \judge \Sigma {\genclient}
                   { \Psi\pp \seq \Gamma, \pair {x}{\quest A} }
          }
          {
            \judge \Sigma {P}
                   { \Psi\pp \seq \Gamma, \pair {x}{A} }
          }
    \\[1ex]
    &\infer[\m{Weaken}]
      {
        \judge \Sigma {\genshutdown}
               { \Psi\pp \seq \Gamma, \pair {x}{{\quest A}} }
      }
      {
        \judge \Sigma {P} { \Psi\pp \seq \Gamma }
      }
    \qquad
    \infer[\m{Contract}]
          {
            \judge \Sigma {\genclone}
                   { \Psi\pp \seq \Gamma, \pair {x}{{\quest A}}}
          }
          {
            \judge \Sigma P
                   { \Psi \pp \seq \Gamma, \pair {x}{{\quest A}}, \pair {x'}{{\quest A}}}
          }
    \\[1ex]
    &\infer[\exists]
      {
        \judge \Sigma{\gensendt}
               { \Psi\pp \seq \Gamma, \pair {x}{\exists X.B} }
      }
      {
        \judge \Sigma P
               { \Psi \pp \seq \Gamma, \pair {x}{B\{A/X\}} &
          X\not\in\m{ftv}(\Psi, \Gamma)}
      }
    \qquad
    \infer[\forall]
          {
            \judge \Sigma {\genrecvt}
                   { \Psi\pp \seq \Gamma, \pair {y}{\forall X.B} }
          }
          {
            \judge \Sigma P
                   { \Psi \pp \seq \Gamma, \pair {y}{B} } &
          X\not\in\m{ftv}(\Psi, \Gamma)
          }
    \\[1ex]
    & \text{no rule for } \nil
    \qquad
    \infer[\top]
          {
            \judge \cdot {\gennocase} {\seq \Gamma, \pair x{\top}}
          }
          {\m{vars}(\Gamma) = \til u}
  \end{eqnarray*}%\normalsize
  % \vspace*{-1.5em}
  \caption{Rules for the Action Fragment}
  %\vspace*{-1.5em}
  \label{fig:mcc_action}
\end{figure*}


==> figures/mcc_equiv_conn.tex <==
\begin{figure*}[!hbt]
  %\scriptsize
\[
\begin{array}{ll@{\!\,\qquad}l}
  [\m{Conn}/\m{Conn}] &
  \hl{(\til  P \pp Q) \pp \til S}
  \equiv \hl{\til P \pp (Q \pp \til S)}&\\[1mm]
  [\m{Conn}/\!\tensor_{1}] & \hl {(\gensend) \pp \til S}
  \equiv \hl {\send{x}{x'}{y',\til z'}{(P\pp \til S)}{Q}} & (\ast)\\[1mm]
  [\m{Conn}/\!\tensor_{2}] & \hl {(\gensend) \pp \til S}
  \equiv \hl {\send{x}{x'}{y',\til z'}{P}{(Q \pp \til S)}} & (\ast)\\[1mm]
  [\m{Conn}/\parr] & \hl{\genrecv \pp \til Q}
  \equiv \hl{\recv {y}{\til x'}{y'}{(P \pp \til Q)}} &\\[1mm]
  [\m{Conn}/\bot] & \hl{\genwait \pp \til Q}
  \equiv \hl{\wait{y}{(P \pp \til Q)}} & \\[1mm]
  [\m{Conn}/\oplus_1] & \hl{\geninl \pp \til Q}
  \equiv \hl{\inl{x}{(P \pp \til Q)} } & \\[1mm]
  [\m{Conn}/\oplus_2] & \hl{\geninr \pp \til Q}
  \equiv \hl{\inr{x}{(P \pp \til Q)} } & \\[1mm]
  [\m{Conn}/\oplus] & \hl{\geninlinr \pp \til S} 
  \equiv \hl{\inlinr{x}{P\pp\til S}{Q\pp\til S}}\\[1mm]
  [\m{Conn}/\with] & \hl{\gencase \pp \til S}
  \equiv \hl{\Case {y}{P \pp \til S}{Q \pp \til S}} & \\[1mm]
  %% [\m{Conn}/!] & \hl{\gensrv \pp \til Q}
  %% \equiv \hl{\srv yx{(P \pp \til Q)} } & \\[1mm]
  [\m{Conn}/?] & \hl{\genclient \pp \til Q}
  \equiv \hl{\client x{\til y}{(P \pp \til Q)}} & \\[1mm]
  [\m{Conn}/\m{Weaken}] & \hl{\genshutdown \pp \til Q}
  \equiv \hl{\shutdown x{\til y}{(P \pp \til Q)}} & \\[1mm]
  [\m{Conn}/\m{Contract}] & \hl{\genclone \pp \til Q}
  \equiv \hl{\clone x{\til y}{x'}{\til y'}{(P \pp \til Q)}} & \\[1mm]
  [\m{Conn}/\exists] & \hl{\gensendt \pp \til Q}
  \equiv \hl{\sendtype x{\til y}A{(P \pp \til Q)}} & (\star)\\[1mm]
  [\m{Conn}/\forall] & \hl{\genrecvt \pp \til Q}
  \equiv \hl{\recvtype yxX{(P \pp \til Q)}} & (\star)\\[1em]
  [\m{Conn}/\Axcut] & \hl{\genaxcut \pp \til Q}
  \equiv \hl{\caxcut{w}{y^B}{x}{(P \pp \til Q)}} &\\[1mm]
  [\m{Conn}/\tensorparr] & \hl{\gencom \pp \til Q}
  \equiv \hl{\com {\til x}{\til x'}{y}{y'}{(P \pp \til Q)}} &\\[1mm]
  %(\til x', y' \not \in \fn{\hl{\til Q}})\\[1mm]
  [\m{Conn}/\onebot] & \hl{\gencomclose \pp \til Q}
  \equiv \hl{\comclose {\til x}y{(P \pp \til Q)}} & \\[1mm]
  [\m{Conn}/\opluswith^{l_1}] & \hl{\genginl \pp \til S}
  \equiv \hl{\comsel{x}{\til y}{\lleft}{(P \pp \til S)}{Q_1,\dots,Q_n}} & (\ast) \\[1mm]
  [\m{Conn}/\opluswith^{l_2}] & \hl{\genginl \pp \til S}
  \equiv \hl{\comsel{x}{\til y}{\lleft}{(P \pp \til S)}{(Q_1, \dots, (Q_i \pp \til S), \dots,Q_n)}} & (\ast) \\[1mm]
  [\m{Conn}/\opluswith^{r_1}] & \hl{\genginr \pp \til S}
  \equiv \hl{\comsel{x}{\til y}{\lright}{P_1,\dots,P_n}{(Q \pp \til S)}} & (\ast) \\[1mm]
  [\m{Conn}/\opluswith^{r_2}] & \hl{\genginr \pp \til S}
  \equiv \hl{\comsel{x}{\til y}{\lright}{(P_1,\dots,(P_i \pp \til S),\dots,P_n)}{(Q \pp \til S)}} & (\ast) \\[1mm]
  [\m{Conn}/\bangwhynot] & \hl{\gengclient \pp \til Q}
  \equiv \hl{\gclient x{\til y}{(P\pp \til Q)}} &(\diamond)\\[1mm]
  [\m{Conn}/\bangw] & \hl{\gengshutdown \pp \til S}
  \equiv \hl{\gshutdown x{\wtil{y(Q)}}{(P \pp \til S)}} & (\diamond) \\[1mm]
  [\m{Conn}/\bangC] & \hl{\gengclone \pp \til Q}
  \equiv \hl{\gclone x{\til y}{x'}{\til y'}{(P \pp \til Q)}} &(\diamond)\\[1mm]
  % (x',\til y' \not \in\fn{\hl{\til Q}} ) \\[1mm]
  [\m{Conn}/\existsforall] & \hl{\gencomt \pp \til Q}
  \equiv \hl{\comtype x{\til y}AX{(P \pp \til Q)}} & (\star)% \\[-1.5em]
\end{array}
\]
%\normalsize
%\caption{Selected commuting conversions, $\m{Conn}$ fragment}
 \caption{Commuting conversions, $\m{Conn}$ fragment}
% \vspace*{-1.5em}
  \label{fig:comconv_conn}
\end{figure*}


==> figures/mcc_equiv_scope.tex <==
\begin{figure*}[!hbt] %\scriptsize
  \[
  \begin{array}{ll@{\!\,\qquad}l}
    [\m{Scope}/\m{Conn}] & \hl{\res {{\til x}:\!G} (P \pp \til Q)} \equiv \hl{\res {{\til x}:G} P \pp \til Q} &\\[1mm]
    [\m{Scope}/\m{Scope}] & \hl{\res {{\til x}:\!G} \res {{\til y}:\!H} P} \equiv \hl{\res {{\til y}:\!H} \res {{\til x}:\!G} P} & \\[1mm]
    [\m{Scope}/\tensor_1 ] & \hl {\res {{\til w}:\! G} (\gensend)} \equiv \hl {\send{x}{x'}{y',\til z'}{ \res{{\til w}:\! G} P}{Q}} & \exists i . w_i \in \m{fv}(P) \\[1mm]
    [\m{Scope}/\tensor_2 ] & \hl {\res {{\til w}:\! G} (\gensend)} \equiv \hl {\send{x}{x'}{y',\til z'}{P}{\res{{\til w}:\! G} Q}} & \exists i. w_i \in \m{fv}(Q)\\[1mm]
    [\m{Scope}/ \parr ] & \hl {\res {{\til w}:\!G} (\genrecv)} \equiv \hl {\recv {y}{\til x'}{y'}{\res {{\til w}:\!G} P}} & \\[1mm]
    [\m{Scope}/ \oplus_1 ] & \hl {\res {{\til w}:\!G} (\geninl)} \equiv \hl {\inl{x}{\res {{\til w}:\!G} P}} & \\[1mm]
    [\m{Scope}/ \oplus_2] & \hl {\res {{\til w}:\!G} (\geninr)} \equiv \hl {\inr{x}{\res {{\til w}:\!G} Q}} & \\[1mm]
    [\m{Scope}/\oplus] & \hl{\res{{\til w}:\!G} (\geninlinr)}
    \equiv \hl{\inlinr{x}{\res{{\til w}:\!G} P}{\res{{\til w}:\!G} Q}}\\[1mm]
    [\m{Scope}/ \with ] & \hl {\res {{\til w}:\!G} (\gencase)} \equiv \hl {\Case {y}{\res {{\til w}:\!G}P}{\res {{\til w}:\!G}Q}} & \\[1mm]
    %% [\m{Scope}/ !] & \hl {\res {{\til w}:\!G} (\gensrv)} \equiv \hl {\srv y x {\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ ? ] & \hl {\res {{\til w}:\!G}(\genclient)} \equiv \hl {\client x {\til y} {\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \m{Weaken} ] & \hl {\res {{\til w}:\!G} (\genshutdown)} \equiv \hl {\shutdown x {\til y} {\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \m{Contract} ] & \hl {\res {{\til w}:\!G} (\genclone)} \equiv \hl {\clone x {\til y}{x'}{\til y'} {\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \exists ] & \hl {\res {{\til w}:\!G} (\gensendt)} \equiv \hl {\sendtype x {\til y} A  {\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \forall ] & \hl {\res {{\til w}:\!G} (\genrecvt)} \equiv \hl {\recvtype y x X {\res {{\til w}:\!G}P}} & \\[1em]
    [\m{Scope}/ \tensorparr ] & \hl {\res {{\til w}:\!G} (\gencom)} \equiv \hl {\com {\til x} {\til x'} y {y'} {\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \onebot ] & \hl {\res {{\til w}:\!G} (\gencomclose)} \equiv \hl {\comclose {\til x}y{\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \opluswith^{l_1} ] & \hl {\res {{\til w}:\!G} (\genginl)}
    \equiv \hl {\comsel{x}{\til y}{\lleft}{\res {{\til w}:\!G}P}{Q_1,\dots,Q_n}} & (\ast)\\[1mm]
    [\m{Scope}/ \opluswith^{l_2} ] & \hl {\res {{\til w}:\!G} (\genginl)}
    \equiv \hl {\comsel{x}{\til y}{\lleft}{\res {{\til w}:\!G}P}{Q_1, \dots,\res {{\til w}:\!G}Q_i, \dots, Q_n}} & (\ast)\\[1mm]
    \m{Scope}/ \opluswith^{r_1} ] & \hl {\res {{\til w}:\!G} (\genginr)}
    \equiv \hl {\comsel{x}{\til y}{\lright}{P_1,\dots,P_n}{\res {{\til w}:\!G}Q}} & (\ast)\\[1mm]
    [\m{Scope}/ \opluswith^{r_2} ] & \hl {\res {{\til w}:\!G} (\genginr)}
    \equiv \hl {\comsel{x}{\til y}{\lright}{P_1,\dots,\res{{\til w}:\!G}P_i,\dots,P_n}{\res {{\til w}:\!G}Q}} & (\ast)\\[1mm]
    [\m{Scope}/\opluswith] & \hl{\res{{\til w}:\!G} (\geninlinr)} \equiv \hl{\inlinr{x}{\res{{\til w}:\!G}P}{\res{{\til w}:\!G}Q}}\\[1mm]
    [\m{Scope}/ \bangwhynot ] & \hl {\res {{\til w}:\!G} (\gengclient)} \equiv \hl {\gclient x{\til y}{\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \bangw ] & \hl {\res {{\til w}:\!G} (\gengshutdown)} \equiv \hl {\gshutdown x{\wtil{y_i(Q_i)}}{\res {{\til w}:\!G}P}} & \\[1mm]
   [\m{Scope}/ \bangC ] & \hl {\res {{\til w}:\!G} (\gengclone)} \equiv \hl {\gclone x{\til y}{x'}{\til y'}{\res {{\til w}:\!G}P}} & \\[1mm]
    [\m{Scope}/ \existsforall ] & \hl {\res {{\til w}:\!G} (\gencomt)} \equiv \hl {\comtype x{\til y}AX{\res {{\til w}:\!G}P}} & \\[-1.5em]
   \end{array} 
    \]%\normalsize
    \caption{Commuting conversions, $\m{Scope}$ fragment}
  %\vspace*{-1.5em}
  \label{fig:comconv_scope}
\end{figure*}


==> figures/mcc_struct.tex <==
\begin{figure}[ht]
  \centering%\scriptsize
  \begin{eqnarray*}
    &\infer[\m{Ax}]
    {
      \judge{\cdot}{\axiom{x}{A}{y}{A^\bot}}{\seq \pair xA, \pair y{A^\bot}}
    }
    {
      A = X \mbox{ or } A = X^\bot 
    }
    \\[1ex]
    &\infer[\m{Conn}]
      {
        \judge{(\Sigma_i)_i, \pair{(x_i)_i}{G}}{(P_i)_i}{\left(\Psi_i \pp \seq \Gamma_i, \pair{x_i}{A_i} 
          \right)_i}
      }
      {
        \left(
        \judge{\Sigma_i}{P_i}{\Psi_i \pp \seq \Gamma_i, \pair{x_i}{A_i}}
        \right)_i
        &
        G \gseq (\pair{x_i}{A_i})_i
      }
      \\[1ex]
    &\infer[\m{Scope}]
      {
        \judge{\Sigma}{\res {{\til x}:G} P}{\Psi \pp \seq \left( \Gamma_i \right)_i}
      }
      {
        \judge{\Sigma, \pair{(x_i)_i}{G}}{P}{\Psi \pp \left(\seq \Gamma_i, \pair{x_i}{A_i} \right)_i}
      }%% \\[1ex]
        %%  &\infer[\m{Plus}]
        %% {\judge{\Sigma}{P + Q}{\Psi}}
        %% {\judge{\Sigma}{P}{\Psi} & \judge{\Sigma}{Q}{\Psi}}
  \end{eqnarray*}%\normalsize
  %\vspace*{-1.5em}
  \caption{Structural Rules}
  % \vspace*{-1.5em}
  \label{fig:mcc_struct}
\end{figure}


==> figures/syntax.tex <==
\begin{figure*}[ht]
% \scriptsize
\begin{align*}
  P ::= & \rule{3mm}{0mm}
  \hl{\axiom{x}{A}{y}{B}}             &&&& \mid \hl{\genaxcut}&& \text{link} \\
%
  & \mid   \hl{ P\pp Q}       &&&&&& \text{parallel composition}\\
  & \mid \hl{\res {{\til x}:G} P}     &&&&&& \text{restriction}\\
  %% & \mid   \hl{ P + Q}       &&&&&& \text{nondeterministic choice}\\
%  & \mid \text{axiom global reduction here? }\\[2mm]
%
  & \mid \hl{\gensend}     &
  & \mid \hl{\genrecv}     &
  & \mid \hl{\gencom}      && \text{communication}\\
%
  & \mid \hl{\genclose}    &
  & \mid \hl{\genwait}     &
  & \mid \hl{\gencomclose} && \text{session close}\\
%
  & \mid \hl{\geninl}      &
  & \mid \hl{\gencase}     &
  & \mid \hl{\genginl}     && \text{left selection}\\
%
  & \mid \hl{\geninr}      &
  &&
  & \mid \hl{\genginr}     && \text{right selection}\\
  & \mid \hl{\geninlinr}   & & & &
  \mid \hl{\genchinlinr} && \text{general selection}\\
%
  & \mid \hl{\genclient}   &
  & \mid \hl{\gensrv}      &
  & \mid \hl{\gengclient}  && \text{server accept/request}\\
%
  & \mid \hl{\genshutdown} &
  &&
  & \mid \hl{\gengshutdown}&& \text{server kill}\\
%
  & \mid \hl{\genclone}    &
  &&
  & \mid \hl{\gengclone}   && \text{server clone}\\
%
  & \mid \hl{\gensendt}    &
  & \mid \hl{\genrecvt}    &
  & \mid \hl{\gencomt}     && \text{type communication}\\
%
  & \mid \hl{\gennocase}   &&&&&& \text{empty choice}
\end{align*}
    % \vspace*{-1.5em}
\begin{align*}
A ::= & \rule{3mm}{0mm}\hl{A\tensor B}       && \text{output} &
  & \mid \hl{A\parr B}        && \text{input} & \qquad
G ::= & \rule{3mm}{0mm}\hl{\gcom {\til x}{y}{G};H}  && (\tensor\parr)\\
%
  & \mid \hl{A\oplus B}       && \text{selection} &
  & \mid \hl{A\with B}             && \text{choice} &
  & \mid \hl{\gsel x{\til y}{G}{H}} && (\oplus\with) \\
%
  & \mid \hl{!A}                  && \text{server} &
  & \mid \hl{?A}             && \text{client} &
  & \mid \hl{\gbang{x}{\til y}{G}}  && (!?) \\
%
  & \mid \hl{\one}              && \text{close} &
  & \mid \hl{\bot}         && \text{wait} &
  & \mid \hl{\gclose{\til x}{y}} && (\one\bot) \\
%
  & \mid \hl{0}          && \text{false} &
  & \mid \hl{\top}             && \text{empty} &
  & \mid \hl{\gabsurd{x}{\til y}}      && (0\top) \\
%
  & \mid \hl{\forall X.A}       && \text{send type} &
  & \mid \hl{\exists X.A} && \text{receive type} &
  & \mid \hl{\gtypecom {X}{x}{\til y}{G}} && (\exists\forall) \\
%
  & \mid \hl{X} && \text{variable} &
  & \mid \hl{X^\bot} && \text{dual variable} &
  & \mid \hl{\globalaxiom{x}{A}{y}{B}}             && (\textsc{axiom})
\end{align*}
% \normalsize
% \vspace*{-2em}
\caption{Syntax of MCC}
% \vspace*{-1em}
\label{fig:mcc_syntax}
\end{figure*}


==> figures/syntax_prog.tex <==
\begin{figure*}[t]
% \scriptsize
\begin{align*}
  P ::= & \rule{3mm}{0mm}
  \hl{\axiom{x}{A}{y}{B}}             &&&& \mid \hl{\genaxcut}&& \text{link} \\
%
  & \mid   \hl{ P\pp Q}       &&&&&& \text{parallel composition}\\
  & \mid \hl{\res {{\til x}:G} P}     &&&&&& \text{restriction}\\
  %% & \mid   \hl{ P + Q}       &&&&&& \text{nondeterministic choice}\\
%  & \mid \text{axiom global reduction here? }\\[2mm]
%
  & \mid \hl{\gensend}     &
  & \mid \hl{\genrecv}     &
  & \mid \hl{\gencom}      && \text{communication}\\
%
  & \mid \hl{\genclose}    &
  & \mid \hl{\genwait}     &
  & \mid \hl{\gencomclose} && \text{session close}\\
%
  & \mid \hl{\geninl}      &
  & \mid \hl{\gencase}     &
  & \mid \hl{\genginl}     && \text{left selection}\\
%
  & \mid \hl{\geninr}      &
  &&
  & \mid \hl{\genginr}     && \text{right selection}\\
  & \mid \hl{\geninlinr}   & & & &
  \mid \hl{\genchinlinr} && \text{general selection}\\
%
  & \mid \hl{\genclient}   &
  & \mid \hl{\gensrv}      &
  & \mid \hl{\gengclient}  && \text{server accept/request}\\
%
  & \mid \hl{\genshutdown} &
  &&
  & \mid \hl{\gengshutdown}&& \text{server kill}\\
%
  & \mid \hl{\genclone}    &
  &&
  & \mid \hl{\gengclone}   && \text{server clone}\\
%
  & \mid \hl{\gensendt}    &
  & \mid \hl{\genrecvt}    &
  & \mid \hl{\gencomt}     && \text{type communication}\\
%
  & \mid \hl{\gennocase}   &&&&&& \text{empty choice}
\end{align*}
% \normalsize
% \vspace*{-2em}
\caption{Syntax of MCC}
% \vspace*{-1em}
\label{fig:mcc_syntax}
\end{figure*}


==> full_example.tex <==
We adapt an example by Carbone and Montesi~\cite{CM13}, where 


=====

\smallpar{Processes and Types.}  Roles $\m{B1}$, $\m{B2}$ and $\m{S}$
from the protocol are implemented as the processes:
\begin{displaymath}\footnotesize
  \begin{array}{l}
    \hl{
    \recv x{\m{B1}}{\m S}{title};\
    \wait{title}{\m{B1}};\
    \send x{\m{B1}}{\m S}{quote};
    \Big(
    \close{quote}{\m{B1}}
    \pp
    \recv x{\m{B1}}{\m{B2}}{contrib};
    \wait{contrib}{\m{B1}};
    \wait x{\m B1};
    \close z{\m Z}
    \Big)
    }
    \\[2mm]
    \hl{
    \send {x}{\m{B2}}{\m S}{quote};\
    \Big(
    \close {quote}{\m{B2}}
    \pp
    \send {x}{\m{B2}}{\m{B1}}{contrib};\
    \big(
    \close {contrib}{\m{B2}}
    \pp
    P_{B2}
    \big)\Big)
    }
    \\[2mm]
    % \hl{\text{Seller}} \DEFEQ
    \hl{
    \send {x}{\m{S}}{\m{B1}}{title};\
    \big(
    \close {title}{\m S}
    \pp
    \recv x{\m{S}}{\m{B1}}{quote};\
    \wait {quote}{\m S};\
    \recv x{\m{S}}{\m{B2}}{quote};\
    \wait {quote}{\m S};\
    \ P_S)\big)
    }
  \end{array}
\end{displaymath}
The first process implements the first buyer $\hl{\text{Buyer1}}$. In
the second process, which implements the second buyer
$\hl{\text{Buyer2}}$, process $\hl{P_{B2}}$ implements the choice of
whether to accept or reject the purchase:
\begin{displaymath}\footnotesize
  \hl{
    \big(\inl {x}{\m {B2} \, \m S};\ 
    % 
    \recv x{\m{B2}}{\m{S}}{addr};\ 
    \wait {addr}{\m S};\
    \close x{\m {B2}} \big)
    % 
    \ \ + \ \
    % 
    \Big(\inr {x}{\m {B2} \, {\m S}}; \close {x}{\m {B2}}
    \Big) 
  }
\end{displaymath}
Finally, in the third process, the implementation of the seller, $P_S$
is the process:
\begin{displaymath}\footnotesize
  \hl {
    {x^{\m S\, \m{B2}}}.\mathsf{case}
    \left(
      \begin{array}{l}
        \send x{\m S}{\m{B2}}{addr};\ 
        \big(\close {addr}{\m S}
        \pp
        \close {x}{\m S}\big),\qquad% \\[1mm]
        \close x{\m S}
      \end{array}
    \right)
  }
\end{displaymath}
At the level of types, the local types in
Example~\ref{ex:2buyerlocaltypes} from \S~\ref{sec:types}
% If we consider the following types: 
% \begin{displaymath}\footnotesize
%   \begin{array}{l}
%     A\DEFEQ \one[\m{B1}]\ \tensor^{\m S}\ 
%     \bot[\m{B1}]\ \parr^{\m S}\
%     \one[\m{B1}]\ \tensor^{\m{B2}}\  \bot
%     \\\\
%     B\DEFEQ \bot[\m{B2}] \ \parr^{\m S}\ \bot[\m{B2}]
%     \,\parr^{\m{B1}}\,   \big((\one[\m{B2}] \tensor^{\m S} \one)
%     \oplus^{\m S} \one \big)
%     \\\\
%     C\DEFEQ
%     \bot[\m S]
%     \ \parr^{\m{B1}}\ 
%     \one[\m S]
%     \tensor^{\m{B1}}
%     \one[\m S]
%     \tensor^{\m{B2}}
%     \Big(
%     (\bot[\m S] \ \parr^{\m{B2}}\ \one)
%     \quad 
%     \with^{\m{B2}}
%     \quad
%     \one
%     \Big)
%   \end{array}
% \end{displaymath}
can be used to type the three processes above, satisfying the
judgements:
% \begin{displaymath}\footnotesize
%   \begin{array}{l}
%
$\hl{\text{Buyer1}}\vdash \pair{x^{\m{B1}}}{A}, \pair{z^{\m Z}}{\one}$,
$\hl{\text{Buyer2}}\vdash \pair{x^{\m{B2}}}{B}$ and
$\hl{\text{Seller}}\vdash \pair{x^{\m S}}{C}$.
%   \end{array}
% \end{displaymath}
If we apply our new cut rule, we obtain
% \begin{displaymath}\footnotesize
$
  \hl{\res {x:G}\big(\text{Buyer1}\ \pp\ \text{Buyer2}\ \pp\
    \text{Seller}\big)}\vdash \pair{z^{\m Z}}{\one}
$
%\end{displaymath}
where the global type $\hl G$, corresponding to equation
(\ref{eq:2buyerproto}) in \S~\ref{sec:preview},
% :
% \begin{displaymath}
%   \begin{array}{l}
%     \gcom{\m{B1}}{\m S}{\gend};\quad 
%     \gcom{\m{S}}{\m{B1}}{\gend};\quad
%     \gcom{\m{S}}{\m{B2}}{\gend};\\
%     \gcom{\m{B1}}{\m{B2}}{\gend};\quad
%     \gsel{\m{B2}}{\m{S}}
%     {
%       \quad \gcom{\m{B2}}{\m{S}}{\gend};\ \gend
%     }
%     {
%       \qquad \gend\quad
%     }
%   \end{array}
% \end{displaymath}
is such that $\hl G\ \gseq\ \pair{\m{B1}}{A},\ \pair{\m{B2}}{B},\ \pair{\m S}{C}$.

\smallskip

\smallpar{Nested Multiparty Sessions.}  We can extend the example
above by implementing the global type (\ref{ciaoMamma}) in
\S~\ref{sec:preview}, where the first buyer creates a sub-session with
the seller if the second buyer decides not to contribute to the
purchase.  Below, we give an excerpt of the new seller:
\begin{displaymath}\footnotesize
  \!\!\!\begin{array}{llll}
    % \hl{\text{Seller}'} \DEFEQ
    \hl{
    \ldots
    \recv x{\!\m{S}}{\m{B1},\m{B2}}{quote};
    \wait{quote}{\m S};
    x^{\m{S}\,\m{B2}}.\mathsf{case}
    \Big(
    \ldots,
    \send x{\m{S}}{\m{B1}}y;
    \big( 
    P_{\m{sub}}
    \pp 
    \send x{\m S}{\m{B1}}{\textit{why}};
    \big(\close{\textit{why}}{\m S}
    \!\pp \!
    \send x{\m S}{\m{B2}}{\textit{why}};
    \ldots
    \big)
    % \wait{\textit{why}}{\m S};
    % \close x{\m S}
    \big) 
    \Big) 
    }
  \end{array}
\end{displaymath}
where $\footnotesize\hl{P_{\m{sub}}} \!= \!
  \hl{
    {y^{\m S\, \m{B1}}}.\mathsf{case}
    \Big(
    \send y{\m S}{\m{B1}}{addr};
    (\close{addr}{\m S} \!\pp\! \close y{\m S}),\quad
    \send y{\m S}{\m{B1}}{\textit{why}};
    (\close{\textit{why}}{\m S} \!\pp\! \close y{\m S})
    \Big)
  }
$.
%
Hence, the type of channel $x$, from the seller's viewpoint, becomes:
\begin{displaymath}\footnotesize
\begin{array}{l}
  \one\tensort{\m{B1}}
  \bot\;\parrt{\m{B1},\m{B2}}\;
  \Big(
  (\one \tensort{\m{B2}} \one)
  \quad
  \witht{\m{B2}}
  \quad 
  \Big( 
  \big( 
  (\one\tensort{\m{B1}}\one) 
  \quad\witht{\m{B1}}\quad
  (\one\tensort{\m{B1}}\one) 
  \big)
  \tensor^{\hl{\m{B1}}}
  \one\tensort{\m{B1}}
  \one\tensort{\m{B2}}
  \one
  \big)
  \Big)
\end{array}
\end{displaymath}
We can then use coherence to infer the global type (\ref{ciaoMamma})
in \S~\ref{sec:preview}.  % Note that after the step of communication,
% the system reduces to
% % $\hl{\res {\pair xG}( ... \pp \res{\pair y{G'}} (...)  )}$, i.e., 
% the composition of two sessions that can be modularly typed using the
% cut rule once per session, as in CLL.

\smallpar{Services.}
We extend the example to support multiple clients on a replicated session $a$:
\begin{displaymath}\footnotesize
  \hl{
    \res{\pair a{\gbang{\m{B1}}{\m{B2},\m S}{G}}}(\ 
    \text{Buyers}
    \pp
    \srv {a^\m{B2}}{x};\text{Buyer2}
    \pp
    \srv {a^\m{S}}{x};\text{Seller}
    \ )
  }
\end{displaymath}
where $\hl{\text{Buyers}}$ is the composition of two buyers: 
$\hl{\res {z:gend}(\, \client {a^\m{B1}}{x};\text{Buyer1} \pp \client
  {a^\m{B1}}{x};\text{Buyer1}' \, )}$.
Process $\hl{\text{Buyer1}'}$ 
initially behaves as $\hl{\text{Buyer1}}$, but we replace $\hl{\close{z}{\m Z}}$ with
$\hl{\wait{z}{\m{Z}}; \close{w}{\m W}}$.
By applying $\beta_{!C}$ once,
$\beta_{!?}$ twice, and commuting conversions, the process above can
be reduced to the parallel composition of two sessions that follow the
2-buyer protocol:
\begin{displaymath}\footnotesize
  \hl{
    \res{\pair x{G}}\Big(
    \text{Buyer2}
    \pp
    \text{Seller}
    \pp
    \res{z:gend}\big( \text{Buyer1} \pp 
    \res{\pair {x}{G}}(
    \text{Buyer2}
    \pp
    \text{Seller}
    \pp
    \text{Buyer1'} )
    \big)
    \Big)
  }
\end{displaymath}
% 
% 
% Using exponentials, we can extend to
% multiple clients (here the first buyer). The new system can start a
% session $a$ obtained with the three processes in the beginning of this
% section:
% \begin{displaymath}\footnotesize
%   \hl{
%     \res{\pair a{\,!G}}\Big(
%     \text{Buyers}
%     \pp
%     \srv {a[\m{B2}]}{x};Buyer2
%     \pp
%     \srv {a[\m{S}]}{x};Seller
%     \Big)
%   }
% \end{displaymath}
% $\hl{\text{Buyers}}$ is the composition of clients, e.g.,
% $\hl{\res {z:\gend}\Big( \client {a[\m{B1}]}{x};Buyer1 \pp \client
%   {a[\m{B1}]}{x};Buyer1' \Big)}$
% in the case of two clients, where $\hl{\text{Buyer1}'}$ is a process
% that initially behaves as $\hl{\text{Buyer1}}$, but such that we replace $\close{z}{\m Z}$ with
% $\wait{z}{\m{Z}}; \close{w}{\m W}$.
% 
% its
% final part is replaced by:
% $\hl{\wait{quote}{\m{B1}}; \close{help}{\m{B1}} \pp \wait {x}{\m
%     {B1}};\ \wait z{\m Z};}$
% $\hl{\close w{\m W}}$.  By applying $(\beta_{!C})$ once,
% $(\beta_{!?})$ twice, and commuting conversions, the process above can
% be reduced to the parallel composition of two sessions that follow the
% 2-buyer protocol:
% \begin{displaymath}\footnotesize
%   \hl{
%     \res{\pair x{G}}\Big(
%     \text{Buyer2}
%     \pp
%     \text{Seller}
%     \pp
%     \res{z:\gend}\big( \text{Buyer1} \pp 
%     \res{\pair x{G}}(
%     \text{Buyer2}
%     \pp
%     \text{Seller}
%     \pp
%     \text{Buyer1'} )
%     \big)
%     \Big)
%   }
% \end{displaymath}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

==> language.tex <==
In this section, we present
%
% a judgemental reconstruction the proof theory
Multiparty Classical Processes (MCP). The key advance of MCP is that
it captures dependencies among actions performed by different
participants in a multiparty session, whereas, in previous work,
actions among different pairs of participants must be
independent~\cite{CP10,W14}.
%
%
% MCP is a conservative extension of the calculus of Classical
% Processes introduced in~\cite{W12} (CP), meaning that terms in MCP
% describing multiparty sessions with only two participants
% corresponds to term in CP. However, in general MCP terms are more
% expressive since they can capture dependencies between actions
% performed by different participants in the same multiparty session.

\smallpar{Environments.}  Let $\Gamma,\Delta$ range over typing
environments of the form:
% 
% associating session names to propositions and roles, where each name
% is distinct:
% \begin{displaymath}
$
\begin{array}{lll}
  \Gamma,\Delta &\ ::=\quad & \cdot\quad | \quad \Gamma, \pair {x^p}A
\end{array}
$.
% \end{displaymath}
Intuitively, $\pair{x^p}{A}$ means that role $\hl p$ in session
$\hl x$ follows behaviour $A$.  We write $?\Delta$ whenever $\Delta$
contains only types of the form $?A$, and write $\Delta,\pair{x^p}{A}$
only when $\hl{x^p}$ does not appear in $\Delta$.

\smallpar{Processes.}  We report the syntax of processes in
Figure~\ref{fig:proc_syntax}.
% 
\begin{figure}[t]
  \begin{displaymath}
    \begin{array}{rrl@{\quad}l@{\quad\qquad}c@{\quad}ll}
      % \textit{Proc.}\quad
      \hl {P,Q,R} & ::=\ 
      & \hl{\recv x{\!p}{\!\tilde q}y;{P}}                   & \textit{(send)} 
      & | & \hl{\send xp{\!q}yPQ}   & \textit{(recv)}            \\[1mm]
      & | & \hl{\inl {x}{pq};P}                  & \textit{(left sel)}
      & | & \hl{\inr {x}{pq};P}              & \textit{(right sel)} \\[1mm]
      & | & \hl{\Case {x}{pq}PQ}          & \textit{(case)}
      & | & \hl{\res {\pair xG} \big(\prod_i P_i\big)}  & \textit{(res)} \\[1mm]
      & | & \hl{\close{x}p}                  & \textit{(close)}    
      & | & \hl{\wait{x}p;P}                 & \textit{(wait)}      \\[1mm]
      & | & \hl{\srv {x^p}y;P}                & \textit{(service)}
      & | & \hl{\client {x^p}y;P }           & \textit{(client)} \\[1mm]
      & | & \hl{P + Q} & \textit{(choice)}
    \end{array}
  \end{displaymath}
  \caption{MCP, syntax of processes.}
  \label{fig:proc_syntax}
\end{figure}
% [IMPROVE]
% Our terms are inspired by the internal $\pi$-calculus, extended with
% multiparty sessions; therefore,
In MCP, both input and output names are bound, as in~\cite{W14}.  Term
\textit{(send)} creates a new session $\hl y$ and sends it, as role
$\hl p$, to the processes respectively playing roles $\hl{\til q}$ in
session $\hl x$;
% interpreting role $p$ in session $x$, willing to perform an output
% to the process interpreting role $q$ in session $x$. The object of
% this output consists of a freshly created session $y$.
then, the process proceeds as $\hl P$.
% Once the output is performed, the process will continue as $P$
% (supposed to communicate on session $y$) and a process $Q$ (supposed
% to continue communicating on session $x$).
The dual operation \textit{(recv)} receives, as role $\hl p$ in
session $\hl x$, a fresh session $\hl y$ from the process playing role
$\hl q$; the process then proceeds as the parallel composition of
$\hl P$ (dedicated to session $\hl y$) and $\hl Q$ (dedicated to
continuing session $\hl x$).  Similarly, terms \textit{(left sel)} and
\textit{(right sel)} multicast a selection of a left or right branch
respectively to the processes playing roles $\hl{\til q}$ in session
$\hl x$, as role $\hl p$. A selection is received by term
\textit{(case)}, which offers the two selectable branches.  Terms
\textit{(close)} and \textit{(wait)} terminate a session.
Term \textit{(choice)} is the standard non-deterministic choice.
In a restriction \textit{(res)}, $\hl x$ is bound in the processes
$\hl{P_i}$; we use the standard type annotation (as in~\cite{W14}) to
show the relation between the semantics of processes and global types
in \S~\ref{sec:semantics}.
In term $\hl{\send xpqyPQ}$, $\hl y$ is
bound in $\hl{P}$ but not in $\hl Q$.
% sends the name $y$ over channel $x$, where the process is playing
% role $p$; then,
In terms $\hl{\recv xp{\tilde q}y{P}}$, $\hl{\srv {x^p}y;P}$, and
$\hl{\client {x^p}y;P}$, $\hl y$ is bound in $\hl P$.

\smallpar{Judgements.}  Judgements in MCP have the form
% \vspace{-5mm}
% \begin{displaymath}
%   \hspace{8cm}
$\hl P \seq \pair{x_1^{p_1}}{A_1},\ldots, \pair{x_n^{p_n}}{A_n}$,
% \end{displaymath}
meaning that process $\hl P$ implements roles $\hl{p_i}$ in the
respective session $\hl{x_i}$ with behaviour $A_i$.
% , respectively for $i\in[1,n]$.

\smallpar{Rules.}  We report the rules of MCP in
Figure~\ref{fig:mcll}.  Intuitively, the behaviour of a process is
typed with local types; then, we use coherence to check that the local
types of composed processes (rule $\m{MCut}$) coherently implement a
global type.
% check that the communications that will be enacted by composing the
% local behaviours of the composed processes correctly implement a
% global scenario.
All rules are defined up to
context exchange.
%
\input{figures/mcll}
% 
% In the remainder of this section, we describe the rules in detail.
%
%\smallpar{The $\m{Cut}$ rule.}  There are two structural rules in
% MCP, the axiom $\m{Ax}$ and the cut rule $\m{Cut}$.

% We comment the rules.
% 
% 
% The axiom of MCP is:
% \begin{displaymath}
%     % \infer[\m{Ax}]
%     {
%       \hl{\fwd{x}{y}}
%       \seq
%       \pair {x}{\wtil{A[p]}},
%       \pair {y}{\wtil{B[q]}}
%     }
%     {
%       \hl G \gseq \wtil{A[p]},\wtil{B[q]}
%     }
% \end{displaymath}
% We interpret $\hl{\fwd{x}{y}}$ as a \emph{multiparty forwader}, meaning that 
% all inputs on $x$ are forwarded as outputs on $y$ and vice versa.
% Therefore, the types of $x$ and $y$ must be coherent.
% 
%Our $\m{Cut}$ rule is an extension of the binary cut from linear logic:
%\begin{displaymath}
%\infer[\m{Cut}]
%    {
%    \hl{\res {\pair xG} \big(\prod_i P_i\big)}
%    \seq
%    \bigcup_i \Delta_i
%    }
%    {
%    \hl{P_i}
%    \seq
%    \Delta_i, \pair x {A_i[p_i]}
%    &
%    \hl G \gseq \wtil{A[p]}
%    }
%\end{displaymath}
Rule $\m{MCut}$ is central to MCP.  It is an extension of the CLL
$\m{Cut}$: instead of just two processes, it allows for the parallel
composition of an arbitrary number of $\hl{P_i}$ that communicate
using session $\hl{x}$. The rule checks that the composition of the
respective local behaviours of the composed processes is coherent
($\hl G \gseq \{\pair {p_i}{A_i}\}_i$). In the conclusion,
$\{\Gamma_i\}_i$ is the disjoint union of all $\Gamma_i$ in the
premise.

% by some role $p$.  The types $\one$ and $\bot$ denote, respectively,
% the request or the acceptance of a channel closing.
%
% The rule for requesting the closure of a channel is:
% \begin{displaymath}
%     \infer[\one]
%    {
%    \hl{\close{x[p]}}
%    \seq
%    \pair x{\one[p]}
%    }
%    {}
%  \end{displaymath}
%
%  In the rule, a process $\hl{\close{x[p]}}$ broadcasts the request
%  for closing a multiparty session $x$, on which it plays role $p$,
%  to all other roles.
%
%  Requests for closing a multiparty session are waited for by the
%  other processes playing a role in the same session:
%  \begin{displaymath}
%    \infer[\bot]
%    {
%    \hl{\wait{x[p]};P}
%    \seq
%    \Delta, \pair x \bot[p]
%    }
%    {
%    \hl P \seq \Delta
%    }
%\end{displaymath}
%Above, a process $\hl{\wait{x[p]};P}$ accepts, as role $p$, to close session 
%$x$ and then proceeds as $\hl P$.
%In the remainder of the paper, for the sake of presentation, we shall
%omit instances of close and wait in our examples.
%
%\subsection{Multiplicatives: Output and Input}
%The multiplicative connectives $\tensor$ and $\parr$ type, respectively, 
%outputs and inputs.
%The rule for outputs is:
%\begin{displaymath}
%    \infer[\tensor]
%    {
%      \hl{\send xpqy{\prod_i P_i}Q}
%      \seq
%      \bigcup_i \Delta_i,\Delta', \pair {x}{(\wtil{A[r]}\tensor^q B)[p]}
%    }
%    {
%      \hl{P_i}
%      \seq 
%      \Delta_i,\pair{y}{A_i[r_i]}
%      &
%      \hl{Q}
%      \seq
%      \Delta',\pair{x}{B[p]}
%    }
%\end{displaymath}

Rule $\tensor$ types an input $\hl{\send xp{\!q}yPQ}$, where the
subprocess $\hl P$ plays role $\hl p$ with behaviour $A$ in the
received multiparty session $\hl y$; session $\hl x$ then proceeds by
following behaviour $B$ for role $\hl p$ in $\hl Q$.  Observe that the
$\tensor$ is annotated with the role $\hl q$ that $\hl p$ wishes to
receive from.
% % and that the local type of the
% % multiparty session $x$ is annotated with the role $p$ played by the
% % process we are typing.
% Above, the processes $\hl{P_i}$ respectively implement behaviour
% $A_i$ for role $r_i$ in session $y$, and process $\hl Q$ implements
% behaviour $B$ for role $p$ on session $x$.  The process
% $\hl{\send xpqy{\prod_i P_i}Q}$ implements the behaviour
% $(\wtil{A[r]}\tensor^q B)[p]$ for role $p$ on channel $x$: it
% creates the fresh name $y$ and sends it to role $q$, and then
% proceeds by executing the processes $\hl{P_i}$ and $\hl Q$ in
% parallel.
%
%The rule for input is:
%\begin{displaymath}
%    \infer[\parr]
%    {
%      \hl{\recv xpqy{P}}
%      \seq
%      \Delta, \pair {x}{ (A[r]\parr^q B)[p]}
%    }
%    {
%      \hl{P}
%      \seq 
%      \Delta,
%      \pair{y}{A[r]},
%      \pair{x}{B[p]}
%    }
%\end{displaymath}
% 
The multicast output $\hl{\recv x{\!p}{\!\tilde q}y;{P}}$ in rule
$\parr$ creates a new session $\hl y$ and sends it, as role $\hl p$ in
session $\hl x$, to roles $\hl{\til q}$.  The new session $\hl y$ is
used by $\hl P$ as role $\hl p$ with type $A$, assuming that the other
processes receiving it implement the other roles (this assumption is
checked by coherence in $\m{MCut}$, when processes are composed).  We
discuss in \S~\ref{sec:related_work} how to relax the constraint that
the role $\hl p$ played in session $\hl y$ is the same.
% %
% % Rule $\parr$ types a multicast output
% % $\hl{\recv x{\!p}{\!\tilde q}y;{P}}$
% % from role $p$ to roles $\til q$
% % checking that the continuation $\hl P$ implements the required
% % behaviours for both sessions $x$ and $y$.
%Process $\hl P$ implements behaviour $A$ for role $r$ on channel $y$ and 
%behaviour $B$ for role $p$ on channel $x$.
%The term $\hl{\recv xpqy{P}}$ implements behaviour
%$(A[r]\parr^q B)[p]$ for role $p$ on channel $x$: it receives the fresh 
%name $y$ from role $p$, and then continues as $\hl P$.

%
%\subsection{Additives: Selection and Branching}
%The additive connectives $\oplus$ and $\with$ are used to type, respectively, 
%the selection from a choice and the offering of a choice.
%
Rules $\oplus_1$ and $\oplus_2$ type, respectively, the multicast of a
left or right selection of a branching, by checking that the process
continuation follows the expected local type.
% There are two rules for selection, denoted by the connective
% $\oplus$, since a process may select from two possible options.  We
% report the rule for left selection (the other is symmetric):
%\begin{displaymath}
%    \infer[\oplus_1]
%    {
%    \hl{\inl {x[p]}{q};P} \seq \Delta, \pair x{(A\oplus^q B)[p]}
%    }
%    {
%    \hl P \seq \Delta,\pair x{A[p]}
%    }
%\end{displaymath}
%Above, process $P$ implements behaviour $A$ for role $p$ on session $x$. Then, 
%process $\hl{\inl {x[p]}{q};P}$ can select the left option offered by role $q$ 
%on session $x$ and proceed as $P$, denoted by the type $(A\oplus^q B)[p]$.
Similarly, rule $\with$ types the offering of two branches
% that can be selected
by checking that the branches implement the respective expected local
types.
%The rule for branching is:
%\begin{displaymath}
%    \infer[\with]
%    {
%    \hl{\Case {x[p]}{q}PQ}
%    \seq
%    \Delta,\pair x{(A \with^q B)[p]}
%    }
%    {
%    \hl P \seq \Delta,\pair x{A[p]}
%    &
%    \hl Q \seq \Delta,\pair x{B[p]}
%    }
%\end{displaymath}
%Above, process $\hl{\Case {x[p]}{q}PQ}$ offers a left and a right choice to 
%role $q$, respectively implemented by process $\hl P$ and $\hl Q$, denoted by 
%the type $(A \with^q B)[p]$.

Rule $+$ types the nondeterministic process $\hl{P + Q}$, by checking
that both $\hl P$ and $\hl Q$ implement the same local
behaviours. Observe that $\hl P$ and $\hl Q$ may still be
substantially different, since they may (i) perform different
selections on some sessions (as rules $\oplus_1$ and $\oplus_2$ can
yield the same typing), and (ii) have different inner compositions of
processes whose types have been hidden by rule $\m{MCut}$.

Rules $\one$ and $\bot$ type, respectively, the request and the
acceptance for closing a multiparty session.
% 
Rules $!$ and $?$ type, respectively, the replicated offering of a
service and its repeated usage (a client).  Since a service typed by
$!$ may be used multiple times, we require that its continuation does
not use any linear behaviour ($?\Delta$).  Rules $\m{Weaken}$ and
$\m{Contract}$ type, respectively, the absence of clients or the
presence of multiple clients. In rule $\m{Contract}$, sessions $\hl y$
and $\hl z$ are contracted into a single session $\hl x$ with a
standard name substitution, provided that they have the same type
$?A$.

\begin{remark}
Removing proof terms from Figure~\ref{fig:mcll} yields a pure logic that
differs from standard CLL only for rule $\m{MCut}$. Since we will prove in \S~\ref{sec:semantics} that $\m{MCut}$ is 
admissible, just like $\m{Cut}$ is admissible in CLL, the two systems subsume the same set of valid 
judgements.
Nevertheless, as shown in the next section, MCP yields a different
operational meaning: reductions of $\m{MCut}$ correspond to multiparty communications, compared to
reductions of $\m{Cut}$ in CLL that correspond to binary communications.
% 
% [ELABORATE,SHORTEN] {\em Removing all (coloured)
%   proof terms from the proof system presented in
%   Figure~\ref{fig:mcll}, yields a pure logic similar to CLL. It is
%   natural to ask how MCP differs from CLL. We observe that MCP and CLL
%   rules differ only in the rules for composition ($\m{Cut}$ in CLL and
%   $\m{MCut}$ in MCP). Since $\m{Cut}$ and $\m{MCut}$ are admissible in
%   CLL and MCP respectively (cf. \S~\ref{sec:semantics} for
%   admissibility of $\m{MCut}$), the two systems prove the same set of
%   propositions. Note that fact that the two systems differ in the rule
%   for composing proofs means that computation (communication) is
%   different, namely more expressive in MCP. In fact, next section is
%   about the semantics of MCP, namely how rule $\m{MCut}$ can be
%   reduced mimicking reductions of processes.}
\end{remark}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> proofsystem.tex <==
Terms of MCC are typed in judgements of the form $\judge\Sigma P\Psi$,
where:
\begin{itemize}
\item $\Sigma$ is a set of session typings of the form
  $\pair{(x_i)_i}{G}$;
\item $P$ is a proof term (a choreography or a process);
\item $\Psi$ is a hypersequent -- a parallel composition of
  classical linear logic sequents.
\end{itemize}
Intuitively, ${\judge\Sigma P\Psi}$ reads as: $\Psi$ types the program
$P$ under the sessions described in $\Sigma$.

Before presenting the typing rules of MCC, we make a few general
remarks.  The notion of hypersequent used in MCC is similar to the one
presented in \cite{CMS18} for intuitionistic linear logic, with a
variation on the treatment of endpoints participating in a session:
instead of marking names that are engaged in a session, we store this
information in $\Sigma$. Given a judgment
$\judge \Sigma P {\Psi \pp \vdash \Gamma, x : A}$,
checking whether $x$ is available and not engaged in a session can be
done by verifying that $x$ does not occur in the domain of
$\Sigma$. It should be noted that names cannot occur more than once in
$\Sigma$: each endpoint $x$ may only belong to (at most) one session
$G$. Hypersequents $\Psi_1, \Psi_2$ and sets of sessions
$\Sigma_1, \Sigma_2$ can only be joined if the names used in their
domains do not repeat.
 
\input{figures/mcc_struct} We divide the typing rules for MCC into
three groups: structural rules, rules for the action fragment and
rules for the interaction fragment. Fig.~\ref{fig:mcc_struct} details
structural rules, which type sessions. Rule~$\m{Ax}$ types a
communication between two processes with dual types. Rules $\m{Conn}$
and $\m{Scope}$ replace the $\m{Cut}$ rule typically found in linear
logic -- and so are best understood as two complementary rules. Read
bottom-to-top, rule~$\m{Scope}$ initiates a session in a choreography,
storing its type in $\Sigma$, while rule~$\m{Conn}$ splits the
choreography of processes involved in a session into parallel,
independent processes.  Rule~$\m{Conn}$ can alternatively be read
top-to-bottom: it merges several independent processes into a joint
session, provided their types are provably coherent -- a notion we
introduce later in this section. When a typing derivation is built
bottom-up, rule $\m{Scope}$ is applied to store a type of a session in
$\Sigma$. The choreography rules (presented below) then destruct the
session type in parallel with the choreography, until the session is
split among its participants by rule $\m{Conn}$.  The types $A_i$ in
that rule are the part of the original session type that has not yet
been ``consumed''.\todo{discuss how conn is deciding, who is talking
  to whom}%% Finally, rule $\m{Plus}$ allows a nondeterministic choice
%% between processes $P$ and $Q$.

\input{figures/mcc_action}

Fig.~\ref{fig:mcc_action} details the rules for typing the action
fragment of MCC, containing its process terms (the first two columns
in Fig.~\ref{fig:mcc_syntax}). In this fragment, we work with
processes not involved in any session -- the endpoints explicitly
mentioned in proof terms can not occur in the domain of $\Sigma$.
These rules do not affect ongoing sessions, except for $\tensor$,
where existing sessions have to be split among the two processes,
combined in the conclusion of the rule. The types for the different
actions follow the intuitions given earlier, the rules themselves
being similar to ones found e.g.~in \cite{CLMSW16,W14}. Notation
$?\Gamma$ means that all endpoint types in $\Gamma$ begin with $?$,
similarly $?\Psi$ requires that all sequents in $\Psi$ are of the form
$?\Gamma$. Processes can only terminate after all their sessions are
closed (so $\Sigma$ is empty).

%% With the exception of generalised $\oplus$, all of these rules are
%% standard. Generalisation of $\oplus$ can in fact be seen as a derived
%% rule, with $\hl \geninlinr$ being a syntactic sugar for $\hl{\geninl +
%%   \geninr}$:
%% \[\footnotesize
%% \infer[\m{Plus}]{\judge{\Sigma}{\geninl + \geninr}{\Psi \pp \seq \Gamma, \pair{x}{A\oplus B}}}
%%       {\infer[\oplus_1]{\judge{\Sigma}{\geninl}{\Psi \pp \seq \Gamma, \pair{x}{A\oplus B}}}
%%         {\judge{\Sigma}{P}{\Psi \pp \seq \Gamma, \pair{x}{A}}} &
%%         \infer[\oplus_2]{\judge{\Sigma}{\geninr}{\Psi \pp \seq \Gamma, \pair{x}{A\oplus B}}}
%%               {\judge{\Sigma}{Q}{\Psi \pp \seq \Gamma, \pair{x}{B}}}}
%% \]

\input{figures/mcc_interaction}

Fig.~\ref{fig:mcc_interaction} details the rules for typing
choreography terms.  At the process level, each of these rules
combines two rules from the action fragment of MCC.  Differently from
the previous set, these rules now also look at $\Sigma$ to check that
the interactions described conform to the types of the ongoing
sessions.  In rule~$\onebot$, we close a session (removed from
$\Sigma$) and terminate all processes involved in it.
Rule~$\tensorparr$ types the creation of a new session with protocol
$G$, created among endpoints $\til z$ and $w$; this session is stored
in $\Sigma$, while the process types are updated as in rules~$\tensor$
and $\parr$ above.  The remaining rules in the linear fragment are
similarly understood. \todo{explain 3 $\opluswith$ rules} Exponentials
give rise to three rules, all of them combining $\bang$ with another
rule.  In rule~$\bangwhynot$, process $x$ invokes the services
provided by $\til y$, creating a new session among these processes
with type $G$.  Rule~$\bangw$ combines $\bang$ with $\m{Weaken}$: here
the processes providing the service are simply removed from the
context.  Rule~$\bangC$ combines $\bang$ with $\m{Contract}$, allowing
a service to be duplicated.  Finally, rule~$\existsforall$ allows $x$
to pass values to parameters in $\til y$, which are then instantiated
by a fresh name $A$ throughout the whole judgement.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> semantics.tex <==
We describe the operational semantics of MCC. As usual, % in process
% calculi where session types are based on linear logic,
this semantics is obtained from cases of the proof of cut elimination:
the principal cases % of cut elimination procedure
describe reductions
($\reducesto$), while the permutations of rule applications % needed for
% the remaining cases
give rise to the rules for structural equivalence
($\equiv$).  We present these rules below, and show that they conform
to the informal semantics described in \S~\ref{sec:cc}.
Following~\cite{CLMSW16,CMS18}, in MCC we split the usual $\m{Cut}$
rule into two components, $\m{Conn}$ and $\m{Scope}$, resulting in
slightly more complex semantics for the $\equiv$ fragment.

\subsection{Reductions}
%
We begin by presenting reductions for both processes and
choreographies.

% We begin by presenting reductions for programs in MCC -- both
% processes and choreographies.

\paragraph{Processes.}
\input{figures/reductions_action}

The semantics of the action fragment of our calculus is presented in
Fig.~\ref{fig:action_semantics}, and follows the intuitions about
process behaviours given in \S~\ref{sec:syntax}. For the sake of
readability, we omit the type annotations from the
restrictions. Notice that the $\beta$-reductions are coordinated by a
global type, as they correspond to multiple parties communicating.%
%% In
%% the first reduction, one for new session creation, the notation $\til
%% x'_{\setminus i}$ denotes $\til x'$ without the component
%% $x'_i$.
\footnote{It may be surprising that some of the rules also
  include a restriction also to a vector $\til z$, and a session
  using a vector of processes $\til S$, whose shape we do not
  inspect. This follows from the shape of coherence rules, described
  in previous section: rules such as $\tensor\parr$, $\oplus\with$,
  $0\top$ and $\exists\forall$ contain an additional context $\Gamma$,
  captured here by $\til z$.}

\todo{Needs changing, does the justification still hold without
  annot.?}  The final two rules in the action fragment make use of the
axiom case of coherence. Note that the reduction can only be applied
directly when the axiom rule is used with type variables. This is
because when the axiom rule uses general types, annotations can be
different. In particular, they may refer to sessions with different
number of endpoints, e.g., $A_1\tensor^x A_2 \parr^y$ and
$A_1\tensor^z A_2 \parr^z$. Therefore, allowing a substitution such as
that of the final two rules may make the resulting term untypable.  As
a consequence, in order to reduce processes we require both the global
type and the linking process to be $\eta$-expanded. Rules for
$\eta$-expanding proof terms in MCC using standard expansion
techniques and for expanding global types are presented in
Fig.~\ref{fig:eta_exp_local}. An alternative way of handling the axiom
cases is to allow both the structural typing rule $\m{Ax}$ and the
coherence axiom, to operate only on type variables, and show
admissibility of the generalized rules as given in
Fig.~\ref{fig:mcc_struct} and Fig.~\ref{fig:coherence}.

\input{figures/eta_expansion}

\paragraph{Choreographies.}
\input{figures/reductions_interaction}

Fig.~\ref{fig:interaction_semantics} defines the semantics for the
interaction fragment of MCC, which again respect the intuitions from
\S~\ref{sec:syntax}. From a proof-theoretical perspective, these
reductions correspond to proof transformations of $\m{C}$-rules from
Fig.~\ref{fig:mcc_interaction} followed by a structural $\m{Scope}$
rule; the transformation removes the $\m{C}$ rule and pushes the
$\m{Scope}$ rule higher up in the proof tree. For instance, in a
choreography for new session creation, the transformation is the
following:
\begin{eqnarray*}
&\infer[\m{Scope}]
      {\judge
        {\Sigma}
        {{\res {\til x^{\til A \tensor \til B}y^{C \parrt{\til x} D} {\til u ^{\til E}} : \gcom{\til x}{y}{G};H} \gencom}}
        {\Psi \pp \seq (\Gamma_{i1}, \Gamma_{i2})_i, \Gamma, (\Gamma_j')_j}}{
\infer[\tensorparr]%\quad (\beta_{\tensor\parr})
      {
        \judge{\Sigma,{\pair{(\til x,y,\til u)}{\gcom{\til x}{y}{G};H}}}
              {{\gencom}}
              {
                \Psi
                \pp
                {( \seq \Gamma_{i1},\Gamma_{i2}, \pair{x_i}{A_i \tensort y B_i} )_i} \pp
                \seq \Gamma, {\pair{y}{C \parrt{\til x} D} \pp
                {( \seq \Gamma'_{j}, \pair{u_j}{E_j} )_j}}
              }
      }
      {\deduce{
        \judge{\Sigma,{\pair{(\til x, y, \til u)}{H},\pair{(\til x',y')}{G\{\til x'/\til x,y'/y\}}}}
              {{P}}
              {
                \Psi
                \pp
                {( \seq \Gamma_{i1}, \pair{x'_i}{A_i} )_i \pp
                  ( \seq \Gamma_{i2}, \pair{x_i}{B_i} )_i} \pp
                \seq \Gamma, {\pair{y'}{C}, \pair{y}{D} \pp
                {( \seq \Gamma'_{j}, \pair{u_j}{E_j} )_j}}
              }
      }{\mathcal{D}}}
      }
\\
&\reducesto
\\
&\infer[\m{Scope}]
      {\judge
        {\Sigma}
        {\res{\til x'^{\til A} y'^{C} : G\{\til x'/\til x,y'/y\}} \res{\til x^{\til B}y^D {\til u^{\til E}} : H} P}
        {\Psi \pp \seq (\Gamma_{i1}, \Gamma_{i2})_i, \Gamma, (\Gamma'_j)_j}
      }
    {\infer[\m{Scope}]
      {\judge{\Sigma,\pair{(\til x',y')}{G\{\til x'/\til x,y'/y\}}}
        {\res{\til x^{\til B}, y^D, {\til u^{\til E}} : H} P}
        {\Psi \pp (\seq \Gamma_{i1}, x'_i:A_i)_i\pp \seq \Gamma,\pair{y'}{C},(\Gamma_{i2})_i,(\Gamma'_j)_j }}
      {\deduce{
        \judge{\Sigma,{\pair{(\til x, y, \til u)}{H},\pair{(\til x',y')}{G\{\til x'/\til x,y'/y\}}}}
              {{P}}
              {
                \Psi
                \pp
                {( \seq \Gamma_{i1}, \pair{x'_i}{A_i} )_i \pp
                  ( \seq \Gamma_{i2}, \pair{x_i}{B_i} )_i} \pp
                \seq \Gamma, {\pair{y'}{C}, \pair{y}{D}\pp
                {( \seq \Gamma'_{j}, \pair{u_j}{E_j} )_j}}
              }
      }{\mathcal{D}}}}
\end{eqnarray*}

\begin{remark}[Server Cloning]\label{rem:clone_inter_sem}$\,$\\
  The reduction rule for a server cloning choreography must clone all
  of the doubled endpoints. Looking at the typing rule $\bangC$ on
  Figure \ref{fig:mcc_interaction}, cloned variables $u_j$ are all of
  the endpoints mentioned in $\left(?\Gamma_i\right)_i$, and $u_j'$
  are corresponding endpoints from $\left(?\Gamma_i'\right)_i$. To
  make the search for these variables syntactic, one could do an
  endpoint projection, as described in the next Section, and look at
  the appropriate subterm of the $\m{Conn}$ rule which connects $y_i$
  and $x$. The $u_j$ are then the free variables of this subterm,
  excluding $y_i$.
\end{remark}

\paragraph{Server Cloning}
When a client process requests a server to clone ($\genclone$), or
when cloning of the server is part of the choreography ($\gengclone$),
the semantic rules governing the execution of such a system have to
ensure certain enpoints get connected at the server-side.

At a proof system level, this is because the weakening in the
exponential fragment is not trace-free. It is worth looking at the
proof transformations that give rise to the semantic rules we have
obtained.\todo{type one or both of the transformations} \todo{explain
  what are the $u_j$s and the $Q'$}
\begin{figure*}
\[
\infer
    {\judge{\Sigma}{\gcpres{x, \til y}{\gbang{x}{\til y}{G}} \genclone \pp (\srv{y_i}{x}{Q_i})_i}{\Psi \pp \seq \Gamma, (?\Gamma_i)_i}}
    {\infer{\judge{\Sigma, (x, \til y) : \gbang{x}{\til y}{G}}{\genclone \pp (\srv{y_i}{x}{Q_i})_i}{\Psi \pp \seq \Gamma, x : ?A \pp (\seq ?\Gamma_i, y_i : !B_i)_i}}
      {\infer{\gbang{x}{\til y}{G} \gseq x: ?A, (y_i: !B_i)_i}{G \gseq x : A, (y_i:B_i)_i} &
        \infer{\judge{\Sigma}{\genclone}{\Psi \pp \seq \Gamma, x : ?A}}
              {\judge{\Sigma}{P}{\Psi \pp \seq \Gamma, x : ?A, x' : ?A}} &
        \left(\infer{\judge{}{\srv{y_i}{x}{Q_i}}{\seq ?\Gamma_i, y_i : !B_i}}
              {\judge{}{Q_i}{\seq ? \Gamma_i, y_i : B_i}}\right)_i
      }}
\]
becomes 
\[
\infer{\judge{\Sigma}{(\cloneo{u_j}{u_j'})_j; \gcpres{x, \til y}{\gbang{x}{\til y}{G}}
        {\gcpres{x', \til y'}{\gbang{x'}{\til y'}{G\{x'/x,\til y'/\til y\}}}
          {P \pp (\srv{y_i}{x}{Q_i})_i} \pp (\srv{y'_i}{x'}{Q_i'})_i}}{\Psi \pp \seq \Gamma, (?\Gamma_i)_i}}
{\infer{\judge{\Sigma}{\gcpres{x, \til y}{\gbang{x}{\til y}{G}}
        {\gcpres{x', \til y'}{\gbang{x'}{\til y'}{G\{x'/x,\til y'/\til y\}}}
          {P \pp (\srv{y_i}{x}{Q_i})_i} \pp (\srv{y'_i}{x'}{Q_i'})_i}}{\Psi \pp \seq \Gamma, (?\Gamma_i)_i, (?\Gamma'_i)_i}}
  {\infer{
      \judge
          {\Sigma, ({x, \til y}) : {\gbang{x}{\til y}{G}}}
          {\gcpres{x', \til y'}{\gbang{x'}{\til y'}{G\{x'/x,\til y'/\til y\}}}
            {P \pp (\srv{y_i}{x}{Q_i})_i} \pp (\srv{y'_i}{x'}{Q_i'})_i}
          {\Psi \pp \seq \Gamma, (?\Gamma'_i)_i, x : ?A \pp (\seq \Gamma_i, y_i:!B_i)_i}}
  {\infer{\judge{\Sigma, (x, \til y) : {\gbang{x}{\til y}{G}}, (x', \til y') : \gbang{x'}{\til y'}{G\{x'/x,\til y'/\til y\}}}
    {{P \pp (\srv{y_i}{x}{Q_i})_i} \pp (\srv{y'_i}{x'}{Q_i'})_i}
    {\Psi \pp \seq \Gamma, x:?A, x':?A \pp (\seq \Gamma_i, y_i : !B_i)_i \pp (\seq \Gamma'_i, y'_i : !B_i)_i }}
    {\infer{\gbang{x}{\til y}{G} \gseq x: ?A, (y_i: !B_i)_i}{G \gseq x : A, (y_i:B_i)_i}
      &
      \infer{\judge{\Sigma, (x', \til y') : {\gbang{x'}{\til y'}{G'}}}{P \pp (\srv{y_i'}{x'}{Q_i'})_i}{\Psi \pp \seq \Gamma, x:?A, x':?A \pp (\seq\Gamma'_i, y_i':!B_i)_i}}
            {\infer{\gbang{x'}{\til y'}{G'} \gseq x': ?A, (y_i': !B_i)_i}{{G'} \gseq x': A, (y_i': B_i)_i}
              & \judge{\Sigma}{P}{\Psi \pp \seq \Gamma, x: ?A, x':?A}
              & \left(\infer{\judge{}{\srv{y_i'}{x'}{Q'_i}}{\seq \Gamma'_i, y'_i : ! B_i}}
                            {\judge{}{Q'_i}{\seq \Gamma'_i, y_i' : B_i}}\right)_i}
      &
      \left(\infer{\judge{}{\srv{y_i}{x}{Q_i}}{\seq \Gamma_i, y_i:!B_i}}
             {\judge{}{Q_i}{\seq \Gamma_i, y_i : B_i}}\right)_i
      }}}}
\]
\hfill with $G' = G\{x'/x, \til y'/\til y\}$, \\
\hfill $\forall j . \exists i . u_j \in \Gamma_i \wedge u'_j \in \Gamma'_i$
\end{figure*}

\subsection{Structural equivalence}

\input{figures/mcc_equiv_conn}
\input{figures/mcc_equiv_scope}

The reductions given earlier require that programs can be written in
the very specific form given in their left-hand side.
Formally, this is achieved by closing $\reducesto$ under structural
equivalence, which we define below: if $P\equiv P'$, $P'\reducesto Q'$
and $Q'\equiv Q$, then $P\reducesto Q$.

The majority of rules for structural equivalence are derived from the
proof of cut-elimination for linear logic. The deconstruction of the
$\m{Cut}$ rule into $\m{Conn}$ and $\m{Scope}$ results in an altered
structural equivalence relation: instead of permuting applications of
$\m{Cut}$ with rules applicable directly before (or after) it in the
proof tree, we have two sets of such permutations---one for $\m{Conn}$
and one for $\m{Scope}$. Intuitively, applications of $\m{Conn}$ and
$\m{Scope}$ have to meet before they can be eliminated. The resulting
structural equivalences, induced by commuting conversions, are
presented in Fig.~\ref{fig:comconv_conn} and
\ref{fig:comconv_scope}. As we are interested only in commuting
conversions of typeable programs, there are certain cases where the
correct equivalence can be found only by looking at the typing
derivation. For instance, a choice between rules
$\m{Conn/\opluswith^{l_1}}$ and $\m{Conn/\opluswith^{l_2}}$ follows
from two possible origins of the endpoint getting connected via
$\m{Conn}$.%% There are two possibilities of handling this ambiguity:
%% either annotate parallel compositions introduced by a $\m{Conn}$ rule
%% with names of endpoints getting connected, allowing to perform a
%% syntactic check on the subprograms, or assert -- as we do here -- that
%% we define these conversions between typeable programs.
The $(\ast)$ side condition in Fig.~\ref{fig:comconv_conn} and
Fig.~\ref{fig:comconv_scope} therefore reads ``provided both sides are
typeable''. In each case precisely one of the available options will
typecheck.
%% Similar ambiguity can be noticed in the
%% $\m{Scope}/\tensor_l$ and $\m{Scope}/\tensor_r$ cases, since in the
%% presence of $\top$ type, we cannot count on all endpoint names being
%% mentioned in the proof term. Again for a syntactic check to be
%% possible, we would need to pollute the $\gennocase$ proof term with
%% the whole context that is being dropped.
Similarly, a potential problem when commuting, e.g. $\m{Conn}$ with
$\exists$ is that the type variable bound by $\exists$ must not occur
in the hyperspequents for any connecting $Q_i$. This can be ensured
using $\alpha$-conversion on type variables, looking at the judgement
in which the term typechecks -- this side condition is marked as
$(\star)$. There always exists an $\alpha-$equivalent proof (and
process).  Finally, we observe that there is no commuting conversion
between $\m{Conn}$ and $\bang $. Indeed, to introduce a $\gensrv$ we need
to know that that nothing is connected to $P$. Therefore, in the
interaction fragment, we only allow this commuting conversion if the
endpoint taking part in the connection originated from a different
sequent, than the endpoint of the server type. This is marked by the
$(\diamond)$ side-condition, and again is a simple check when looking
at the typing judgment. Of course, in order to obtain a deadlock
freedom result, we need to have some commuting conversion for
$\gensrv$ -- it is, for this system, a slightly unusual one, as we
commute $\bang $ introduction past both $\m{Conn}$ and $\m{Scope}$:
\[
\infer{\judge{}{\res{{\til x x}:\!G}(\gensrv \pp \til Q)}{\seq \quest \Gamma, \left(\quest \Gamma_i\right)_i, \pair y{\bang A}}}
      {\infer{\judge{\pair{(\til x, x)}{G}}{\gensrv \pp \til Q}{\seq \Gamma, \pair x{\quest B}, \pair y{\bang A} \pp \left( \seq \quest \Gamma_i, \pair{x_i}{B_i}\right)_i}}
        {\infer{\judge{}{\gensrv}{\seq \quest \Gamma, \pair x{\quest B}, \pair y{\bang A}}}
          {\judge{}{P}{\seq \quest \Gamma, \pair x{\quest B}, \pair y A}}&
          \left(\judge{}{Q_i}{\seq \quest \Gamma_i, \pair{x_i}{B_i}}\right)_i& G \gseq \left(\pair{x_i}{B_i} \right)_i, \pair{x}{\quest B}}}
\]
becomes
\[
\infer{\judge{}{\srv{y}{}{\res{{\til x x}:\!G}(P \pp \til Q)}}{\seq \quest \Gamma, \left(\quest \Gamma_i\right)_i, \pair y{\bang A}}}
      {\infer{\judge{}{\res{{\til x x}:\!G}(P \pp \til Q)}{\seq \quest \Gamma, \left(\quest \Gamma_i\right)_i, \pair y{A}}}
        {\infer{\judge{\pair{(\til x, x)}{G}}{P \pp \til Q}{\seq \Gamma, \pair x{\quest B}, \pair y{A} \pp \left( \seq \quest \Gamma_i, \pair{x_i}{B_i}\right)_i}}
        {\judge{}{P}{\seq \quest \Gamma, \pair x{\quest B}, \pair y A}&
          \left(\judge{}{Q_i}{\seq \quest \Gamma_i, \pair{x_i}{B_i}}\right)_i& G \gseq \left(\pair{x_i}{B_i} \right)_i, \pair{x}{\quest B}}}}
      \]
This gives rise to a commuting conversion
\[
\res{{\til x x}:\!G}(\gensrv \pp \til Q) \equiv \srv{y}{}{\res{{\til x x}:\!G}(P \pp \til Q)}
\]
-- but only in the case when a connection is made with processes which
are not connected to anything, and whose endpoints are of $\quest$
type. This is enough for our purposes, and is in fact a generalization
of the standard commuting conversion for $\bang$, as found in
\cite{W14}. In the interaction fragment we require the same of the
connecting $Q_i$s, giving rise to the commuting conversion
\[
\res{{\til z z}:\!G}(\gengclone \pp \til Q) \equiv \gclone x{\til y}{x'}{\til y'}{\res{{\til z z}:\!G}(P\pp\til Q)}
\]

A similar situation arises when considering $\top$: we can only
permute $\top$ with both $\m{Conn}$ and $\m{Scope}$ at once, and only
if the connecting processes are themselves not connected to
anything. This is consistent with the process interpretation: within
this session, an empty choice is offered, forcing the communication to
cease.

\[
\infer{\judge{}{\res{{\til z,z}:\!G}{(\nocase{x}{}{\til u, z}\pp \til Q)}}{\seq \Gamma, \left(\Gamma_i\right)_i, \pair{x}{\top}}}
      {\infer{\judge{\pair{(\til z, z)}{G}}{\nocase{x}{}{\til u, z}\pp \til Q}{\seq \Gamma, \pair{x}{\top}, \pair{z}{B} \pp \left(\seq \Gamma_i, \pair{z_i}{B_i} \right)_i}}
        {\infer{\judge{}{\nocase{x}{}{\til u, z}}{\seq \Gamma,\pair{z}{B},\pair{x}{\top}}}
          {\m{vars}(\Gamma) = \til u} &
          \left(\judge{}{Q_i}{\seq \Gamma_i, \pair{z_i}{B_i} \right)_i &
            G \gseq \left(\pair{z_i}{B_i}\right)_i, \pair{z}{B}}}}
\]
becomes
\[
\infer{\judge{}{\nocase{x}{}{\til u, \til v}}{\seq \Gamma, \left(\Gamma_i\right)_i, \pair{x}{\top}}}
{\m{vars}(\Gamma) = \til u & \left(\m{vars}(\Gamma_i)\right)_i = \til v}
\]

This corresponds to the commuting conversion
\[
\res{{\til z,z}:\!G}{(\nocase{x}{}{\til u, z}\pp \til Q)} \equiv {\nocase{x}{}{\til u, \til v}}
  \qquad\qquad \mbox{ where }\til v = \left(\m{vars}((Q_i)\right)_i \setminus \til z
  \]
  
Besides the commuting conversions above, we also have the usual
structural equivalence rules, making the parallel composition under
restriction, the linking process and the global type for linking
sessions symmetric. Furthermore, the order of restrictions can be
swapped.

\begin{align*}
  \hl{\axiom x A y B} & \equiv \hl{\axiom y {A^\bot} x A}
  \\
  \hl{\gcpres{\til w, y, x, \til z}{G}{\til P \pp R \pp Q \pp \til S}} 
  &\equiv \hl{\gcpres{\til w, x, y, \til z}{G}{\til P \pp Q \pp R \pp \til S}}
  \\
  \hl{\gcpres{z, \til w}{H}{\gcpres{x, \til y}{G}{P \pp \til R} \pp \til Q}}
  &\equiv 
  \phl{\gcpres{x, \til y}{G}{\gcpres{z, \til w}{H}{P \pp \til Q} \pp \til R}}
\end{align*}

\subsection{Properties}

This simple lemma justifies the shape of reductions in $\m{Weaken}$
and $\m{Contract}$ cases.
\begin{lemma}$\;$\\
$\judge{\Sigma}{\Psi}{P}$ and $x \in \m{vars}(\Psi)$ implies that $x \in \m{fv}(P)$ 
\end{lemma}


As structural congruence is typing-based, with side conditions
($\ast$), ($\star$) and ($\diamond$) posing requirements on the
connection and scoping, we can establish subject congruence.

\begin{property}[Subject Congruence]$\;$\\
  $\judge \Sigma P \Psi$ and $P \equiv Q$ implies that
  $\judge \Sigma Q \Psi$.
\end{property}

Furthermore, since the reductions in our system are based on proof
transformations, they preserve typing. In the next result,
$\reducestom$ is the reflexive transitive closure of the reduction
relation $\reducesto$, which may use commuting conversions as defined
on Fig.~\ref{fig:comconv_conn} and Fig.~\ref{fig:comconv_scope}.

\begin{theorem}[Subject Reduction]$\,$\\
  $\judge \Sigma P \Psi$ and $P \reducestom Q$ implies $\judge \Sigma
  Q \Psi$.
\end{theorem}

Finally, we can show that MCC is deadlock-free by arguing that the
top-level $\m{Scope}$ application can be pushed up the
derivation. Proof theoretically, this procedure can be viewed as MCC's
equivalent of the Principal Lemma of Cut Elimination.
% Can we do a direct proof? If not, should the indirect one (with
% translation to CP) be given in the appendix?

\begin{theorem}[Deadlock-freedom]\label{thm:deadlockfree}$\,$\\
$\judge \Sigma P \Psi$ implies that there exists $Q$ such that $P
  \reducestom Q$ and $Q$ is not $\m{Scope}$.
\end{theorem}

%% Finally, by persistently applying commuting conversions in order to
%% allow triggering reductions, we can eventually reach a proof term
%% which is free of applications of $\m{Scope}$ rule. Proof
%% theoretically, this procedure can be viewed as MCC's equivalent of a
%% cut elimination theorem: $\m{Scope}$ elimination.


%% \begin{theorem}[Termination/Deadlock-freedom]\label{thm:deadlockfree}$\,$\\
%%   $\judge \Sigma P \Psi$ implies that there exists $Q$ which is
%%   \emph{restriction-free} and such that $P\reducestom Q$ and $\judge
%%   \Sigma Q \Psi$.
%% \end{theorem}



% 
%
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

